CARMENES input catalogue of M dwarfs IX. Multiplicity from close spectroscopic binaries to ultra-wide systems

Multiplicity studies greatly benefit from focusing on M dwarfs because they are often paired in a variety of configurations with both stellar and substellar objects, including exoplanets. We aim to address the observed multiplicity of M dwarfs by conducting a systematic analysis using the latest available astrophotometric data. For every star in a sample of 2214 M dwarfs from the CARMENES catalogue, we investigated the existence of resolved and unresolved physical companions in the literature and in all-sky surveys, especially in Gaia DR3 data products. We covered a very wide range of separations, from known spectroscopic binaries in tight arrangements $\sim$0.01 au to remarkably separated ultra-wide pairs ($\sim$10$^5$ au). We identified 835 M dwarfs in 720 multiple systems, predominantly binaries. Thus, we propose 327 new binary candidates based on Gaia data. If these candidates are finally confirmed, we expect the multiplicity fraction of M dwarfs to be 40.3$^{+2.1}_{-2.0}$ %. When only considering the systems already identified, the multiplicity fraction is reduced to 27.8$^{+1.9}_{-1.8}$ %. This result is in line with most of the values published in the literature. We also identified M-dwarf multiple systems with FGK, white dwarf, ultra-cool dwarf, and exoplanet companions, as well as those in young stellar kinematic groups. We studied their physical separations, orbital periods, binding energies, and mass ratios. We argue that based on reliable astrometric data and spectroscopic investigations from the literature (even when considering detection biases), the multiplicity fraction of M dwarfs could still be significantly underestimated. This calls for further high-resolution follow-up studies to validate these findings.

==> tables/figures_light_curves.tex <==
\begin{figure*}[]
    \begin{subfigure}{\linewidth}
	\includegraphics[width=0.49\linewidth]{plot_light_curve_750.pdf}
	\includegraphics[width=0.49\linewidth]{plot_light_curve_837.pdf}
    \end{subfigure}
    \begin{subfigure}{\linewidth}
    \includegraphics[width=0.49\linewidth]{plot_light_curve_961.pdf}
    \includegraphics[width=0.49\linewidth]{plot_light_curve_1056.pdf}  
    \end{subfigure}
	\begin{subfigure}{\linewidth}
    \includegraphics[width=0.49\linewidth]{plot_light_curve_1181.pdf}
    \includegraphics[width=0.49\linewidth]{plot_light_curve_1286.pdf}
    \end{subfigure}
    \caption{Same as Fig.~\ref{fig:light_curve} for single stars reported in this work as unresolved binary candidates.}
     \label{fig:light_curves_appendix}
\end{figure*}
\clearpage
\begin{figure*}[]
    \ContinuedFloat
    \begin{subfigure}{\linewidth}
	\includegraphics[width=0.49\linewidth]{plot_light_curve_1669.pdf}
	\includegraphics[width=0.49\linewidth]{plot_light_curve_2011.pdf}
    \end{subfigure}
    \begin{subfigure}{\linewidth}
    \includegraphics[width=0.49\linewidth]{plot_light_curve_2623.pdf}
    \includegraphics[width=0.49\linewidth]{plot_light_curve_2502.pdf}  
    \end{subfigure}
	\begin{subfigure}{\linewidth}
    \includegraphics[width=0.49\linewidth]{plot_light_curve_2517.pdf}
    \includegraphics[width=0.49\linewidth]{plot_light_curve_2560.pdf}
    \end{subfigure}
    \caption{Same as Fig.~\ref{fig:light_curve} for the single stars reported in this work as candidates to unresolved binaries (cont.).}
\end{figure*}

==> tables/table_EB.tex <==
\begin{table}
\footnotesize
\caption{Eclipsing binaries in our sample$^a$.}
\label{tab:eclipsing} 
\centering
\begin{tabular}{lccccc}
    \hline\hline 
    \noalign{\smallskip}  
&	GJ 3236			&	Castor C			&	CU Cnc			&	LP 177--102			&	CM Dra			\\
\hline
\noalign{\smallskip}
\noalign{\smallskip}																		
Karmn	&	J03372+691			&	J07346+318			&	J08316+193S			&	J15474+451			&	J16343+571			\\
\noalign{\smallskip}																					
$\mathcal{M}_1$ {[}$\mathcal{M}_\odot${]}	&	0.376	 $\pm$ 	0.017	&	0.5992	 $\pm$ 	0.0047	&	0.4349	 $\pm$ 	0.0012	&	0.2576	 $\pm$ 	0.0085	&	0.23102	 $\pm$ 	0.00089	\\
\noalign{\smallskip}																					
$\mathcal{M}_2$ {[}$\mathcal{M}_\odot${]}	&	0.281	 $\pm$ 	0.015	&	0.5992	 $\pm$ 	0.0047	&	0.39922	 $\pm$ 	0.00089	&	0.2585	 $\pm$ 	0.0080	&	0.21409	 $\pm$ 	0.00083	\\
\noalign{\smallskip}																					
$\mathcal{R}_1$ {[}$\mathcal{R}_\odot${]}	&	0.3828	 $\pm$ 	0.0070	&	0.6191	 $\pm$ 	0.0057	&	0.4323	 $\pm$ 	0.0055	&	0.2895	 $\pm$ 	0.0068	&	0.2534	 $\pm$ 	0.0019	\\
\noalign{\smallskip}																					
$\mathcal{R}_2$ {[}$\mathcal{R}_\odot${]}	&	0.2992	 $\pm$ 	0.0075	&	0.6191	 $\pm$ 	0.0057	&	0.3916	 $\pm$ 	0.0094	&	0.2895	 $\pm$ 	0.0068	&	0.2398	 $\pm$ 	0.0018	\\
\noalign{\smallskip}																					
$P_{\rm orb}$ {[}d{]}	&	0.7712600	 $\pm$ 	0.0000023	&	0.8142822	 $\pm$ 	0.0000010	&	2.771468	 $\pm$ 	0.000004	&	3.5500184	 $\pm$ 	0.0000018	&	1.268389985	 $\pm$ 	0.000000005	\\
\noalign{\smallskip}																					
$a$ {[}au{]}	&	0.01430			&	0.01819			&	0.03624			&	0.03654			&	0.01750			\\
\noalign{\smallskip}																					
Reference	&	{Irw09, Shk10}			&	{Joy26, Giz02, Tor22}			&	{Del99a, Del99b, Tor10}			&	{Moc02, Har11, Bir12}			&	{Mor09, Tor10, Scha19}			\\
\noalign{\smallskip}
\hline
\end{tabular}
\tablefoot{
\tablefoottext{a}{
\,\,Bir12	: \cite{Bir12};
Del99a: \cite{Del99a};
Del99b: \cite{Del99b};
Giz02: \cite{Giz02};
Har11: \cite{Har11};
Irw09: \cite{Irw09};
Joy26: \cite{Joy26};
Moc02: \cite{Moc02};
Mor09: \cite{Mor09};
Scha19: \cite{Scha19};
Shk10: \cite{Shk10};
Tor10: \cite{Tor10};
Tor22: \cite{Tor22}.}   
}
\end{table}

==> tables/table_FGK.tex <==

{\fontsize{7}{10}\selectfont 
\begin{landscape}
\begin{longtable}{lllllccclcc}
\caption{\label{tab:fgk} Multiple systems containing M dwarfs and FGK primaries.}
\\
\noalign{\smallskip}
\noalign{\smallskip}
\noalign{\smallskip}
\hline\hline
\noalign{\smallskip}
Name	&	Karmn	&	Spectral	&	Component	&	Discoverer$^a$	&	$\pi$			&	$\mu_{\rm total}$			&	[Fe/H]	&	[Fe/H]	&	$\rho$	&	$\theta$	\\
	&		&	type	&		&		&	{[}mas{]}			&	{[}mas\,a$^{-1}${]}			&	{[}dex{]}	&	Ref.$^b$	&	{[}arcsec{]}	&	{[}deg{]}	\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
\endfirsthead
\caption{Multiple systems containing M dwarfs and FGK primaries (cont.).}\\
\hline\hline
        \noalign{\smallskip}
Name	&	Karmn	&	Spectral	&	Component	&	Discoverer$^a$	&	$\pi$			&	$\mu_{\rm total}$			&	[Fe/H]	&	[Fe/H]	&	$\rho$	&	$\theta$	\\
	&		&	type	&		&		&	{[}mas{]}			&	{[}mas\,a$^{-1}${]}			&	{[}dex{]}	&	Ref.$^b$	&	{[}arcsec{]}	&	{[}deg{]}	\\
\hline
\noalign{\smallskip}
\endhead
%
\hline
\endfoot
\noalign{\smallskip}
HD 4967	&		&	K5 V	&	A	&		&	65.090	$ \pm $	0.025	&	672.691	$ \pm $	0.047	&	--0.33	&	Hou16	&		&		\\
HD 4967 B	&	J00515--229	&	M5.5 V	&	B	&	LDS 1082	&	65.073	$ \pm $	0.050	&	680.566	$ \pm $	0.095	&	\ldots	&		&	17.07	&	72.1	\\
\noalign{\smallskip}        \noalign{\smallskip}																									
EX Cet	&		&	K0.5 V	&	A	&		&	41.564	$ \pm $	0.024	&	197.856	$ \pm $	0.032	&	--0.06	&	Zak22	&		&		\\
LP 648--20	&	J01369--067	&	M3.5 V	&	B	&	CAB 3	&	41.699	$ \pm $	0.045	&	200.547	$ \pm $	0.052	&	\ldots	&		&	612.08	&	258.6	\\
\noalign{\smallskip}        \noalign{\smallskip}																									
Wolf 109	&		&	K5 V	&	A	&		&	27.827	$ \pm $	0.021	&	466.135	$ \pm $	0.031	&	\ldots	&		&		&		\\
Wolf 109 B	&	J02020+039	&	M2.0 V	&	B	&	OSV 1	&	28.922	$ \pm $	0.353	&	465.771	$ \pm $	0.482	&	\ldots	&		&	17.96	&	14.4	\\
G3 2517912315149114240	&		&	M5.0 V	&	C	&		&		\ldots		&		\ldots		&		&		&	17.74	&	16.8	\\
\noalign{\smallskip}        \noalign{\smallskip}																									
HD 15468	&		&	K4.5 V	&	AB	&	RST 2280	&	51.606	$ \pm $	0.136	&	646.402	$ \pm $	0.166	&	--0.31	&	Mon18	&	0.18	&	145.3	\\
GJ 100 C	&	J02285--200	&	M2.5 V	&	C	&	UC 744	&	50.972	$ \pm $	0.032	&	649.191	$ \pm $	0.038	&	0.14	&	Kuz19	&	474.57	&	242.1	\\
\noalign{\smallskip}        \noalign{\smallskip}																									
HD 16160	&		&	K3 V	&	AB	&	GKI 1	&	138.340	$ \pm $	0.318	&	2312.099	$ \pm $	0.496	&	--0.09	&	Tin19	&	1.73	&	289.5	\\
BX Cet	&	J02362+068	&	M4.0 V	&	C	&	PLQ 32	&	138.437	$ \pm $	0.042	&	2312.992	$ \pm $	0.057	&	--0.24	&	Marf21	&	164.25	&	318.4	\\
\noalign{\smallskip}        \noalign{\smallskip}																									
HD 16895	&		&	F8 V	&	A	&		&	89.685	$ \pm $	0.164	&	346.403	$ \pm $	0.244	&	0.04	&	Mon18	&		&		\\
GJ 107 B	&	J02441+492	&	M1.5 V	&	B	&	STF 296	&	89.374	$ \pm $	0.032	&	322.947	$ \pm $	0.042	&	\ldots	&		&	20.93	&	305.1	\\
\noalign{\smallskip}        \noalign{\smallskip}																									
HD 18143 A	&		&	K2 IV	&	A	&		&	44.432	$ \pm $	0.021	&	327.700	$ \pm $	0.032	&	0.17	&	Ros21	&		&		\\
HD 18143 B	&		&	K7 V	&	B	&	STF 326	&	44.505	$ \pm $	0.025	&	327.976	$ \pm $	0.042	&	0.14	&	Gai14b	&	4.78	&	221.3	\\
HD 18143 C	&	J02555+268	&	M4.0 V	&	C	&	LDS 883	&	44.522	$ \pm $	0.023	&	328.058	$ \pm $	0.035	&	\ldots	&		&	43.79	&	266.3	\\
\noalign{\smallskip}        \noalign{\smallskip}																									
HD 18757	&		&	G1.5 V	&	A	&		&	42.459	$ \pm $	0.020	&	1000.787	$ \pm $	0.023	&	--0.23	&	Hir21	&		&		\\
GJ 3195	&	J03047+617	&	M3.0 V	&	B	&	LDS 9142	&	42.534	$ \pm $	0.026	&	1000.094	$ \pm $	0.033	&	\ldots	&		&	263.30	&	65.8	\\
\noalign{\smallskip}        \noalign{\smallskip}																									
V577 Per	&		&	K2 V	&	A	&		&	27.482	$ \pm $	0.031	&	188.424	$ \pm $	0.039	&	--0.09	&	Mon18	&		&		\\
HD 21845 B	&	J03332+462	&	M0.0 V	&	B	&	ES 560	&	27.481	$ \pm $	0.016	&	185.831	$ \pm $	0.021	&	\ldots	&		&	9.50	&	142.3	\\
\noalign{\smallskip}        \noalign{\smallskip}																									
HD 278874	&		&	K2 V	&	Aab	&	Mon18	&	25.434	$ \pm $	0.032	&	36.209	$ \pm $	0.044	&	\ldots	&		&		&		\\
HD 278874 B	&	J03397+334	&	M3.0 V	&	B	&	ES 327	&	25.571	$ \pm $	0.041	&	38.831	$ \pm $	0.061	&	\ldots	&		&	15.47	&	294.3	\\
\noalign{\smallskip}        \noalign{\smallskip}																									
HD 23189	&		&	K2 V	&	A	&	KUI 13	&	55.825	$ \pm $	0.013	&	279.831	$ \pm $	0.016	&	--0.43	&	Hou16	&		&		\\
GJ 153 C	&	J03480+686	&	M1.5 V	&	BC	&	KUI 13	&	55.984	$ \pm $	0.105	&	288.831	$ \pm $	0.215	&	\ldots	&		&	13.20	&	17.2	\\
\noalign{\smallskip}        \noalign{\smallskip}																									
HD 275867	&		&	K2 V	&	A	&		&	30.985	$ \pm $	0.016	&	62.067	$ \pm $	0.023	&	--0.13	&	Mon18	&		&		\\
TYC 2868--639--1	&	J03519+397	&	M0.0 V	&	B	&	GRV 197	&	31.021	$ \pm $	0.020	&	64.399	$ \pm $	0.026	&	\ldots	&		&	53.92	&	207.5	\\
\noalign{\smallskip}        \noalign{\smallskip}																									
HD 24916	&		&	K4 V	&	A	&		&	65.426	$ \pm $	0.023	&	234.331	$ \pm $	0.031	&	0.09	&	Ros21	&		&		\\
HD 24916 B	&	J03574--011	&	M2.5 V	&	Bab	&	Zak79 / BU 543	&	65.492	$ \pm $	0.044	&	251.747	$ \pm $	0.057	&	0.01	&	Kuz19	&	14.13	&	11.0	\\
\noalign{\smallskip}        \noalign{\smallskip}																									
o$^{02}$ Eri B	&		&	DA2.9	&	A	&		&	199.691	$ \pm $	0.051	&	4018.591	$ \pm $	0.061	&		&		&		&		\\
o$^{02}$ Eri	&		&	K0 V	&	B	&	STF 518	&	199.608	$ \pm $	0.121	&	4089.836	$ \pm $	0.165	&	--0.20	&	Ros21	&	83.34	&	102.2	\\
o$^{02}$ Eri C	&	J04153--076	&	M4.5 V	&	C	&	STF 518	&	199.452	$ \pm $	0.069	&	4083.715	$ \pm $	0.084	&	--0.30	&	Marf21	&	78.10	&	97.5	\\
\noalign{\smallskip}        \noalign{\smallskip}																									
TYC 78--257--1	&		&	$\sim$K3.0 V	&	A	&		&	26.974	$ \pm $	0.022	&	139.559	$ \pm $	0.028	&	--0.06	&	Boc18	&		&		\\
RX J0422.4+0337	&	J04224+036	&	M3.5 V	&	B	&	Sma21	&	27.846	$ \pm $	0.026	&	143.007	$ \pm $	0.039	&	0.39	&	Ter15a	&	1748.61	&	43.9	\\
\noalign{\smallskip}        \noalign{\smallskip}																									
HD 27848	&		&	F5 V	&	AB	&	OCC 615	&	19.959	$ \pm $	0.026	&	103.388	$ \pm $	0.039	&	--0.11	&	Bud21	&		&		\\
V991 Tau	&		&	K4 V	&	C	&		&	18.356	$ \pm $	0.019	&	94.411	$ \pm $	0.025	&	0.19	&	Bud21	&	641.17	&	121.9	\\
V805 Tau	&	J04252+172	&	M3.5 V	&	DE	&	AST 4	&	19.313	$ \pm $	0.193	&	110.653	$ \pm $	0.259	&	\ldots	&		&	1002.15	&	47.1	\\
LP  415--881	&		&	M7.0 V	&	F	&		&	21.204	$ \pm $	0.061	&	105.698	$ \pm $	0.088	&	\ldots	&		&	1677.61	&	93.4	\\
\noalign{\smallskip}        \noalign{\smallskip}																									
V583 Aur	&		&	K5 V	&	A	&		&	11.128	$ \pm $	0.018	&	52.345	$ \pm $	0.027	&	\ldots	&		&		&		\\
PM J04393+3331	&	J04393+335	&	M4.0 V	&	BC	&	JNN 263	&	7.425	$ \pm $	0.848	&	50.282	$ \pm $	1.831	&	0.10	&	Ter15a	&	207.05	&	61.9	\\
\noalign{\smallskip}        \noalign{\smallskip}																									
HD 31412	&		&	F9.5 V	&	AB	&	EGN 4	&	27.865	$ \pm $	0.027	&	233.457	$ \pm $	0.035	&	0.04	&	Ros21	&	0.44	&	17.7	\\
HD 31412 B	&	J04559+046	&	M2.0 V	&	C	&	LDS 9181	&	27.851	$ \pm $	0.026	&	233.996	$ \pm $	0.034	&	\ldots	&		&	21.66	&	277.9	\\
	\noalign{\smallskip}        \noalign{\smallskip}																								
Capella	&		&	G3 III	&	Aab	&	She85 / Tor09	&	76.200	$ \pm $	0.460	&	433.472	$ \pm $	0.608	&	--0.37	&	Mas08	&		&		\\
Capella H	&	J05173+458	&	M2.5 V	&	B	&	FRH  	&	74.952	$ \pm $	0.019	&	437.931	$ \pm $	0.026	&	\ldots	&		&	722.84	&	141.8	\\
Capella L	&		&	M4.0 V	&	C	&	ST 3	&	75.184	$ \pm $	0.053	&	420.381	$ \pm $	0.077	&	\ldots	&		&	3.46	&	173.5	\\
\noalign{\smallskip}        \noalign{\smallskip}																									
HD 35956	&		&	G0 V	&	Aab	&	Kat13	&	33.788	$ \pm $	0.294	&	231.784	$ \pm $	0.417	&	0.28	&	Ric20	&		&		\\
HD 35956 B	&		&	M1.0 V	&	B	&	TOK 94	&	35.405	$ \pm $	0.020	&	237.813	$ \pm $	0.029	&	\ldots	&		&	5.83	&	71.4	\\
G 102--4 A	&	J05289+125	&	M4.0 V	&	C	&	LDS 6186	&	39.500	$ \pm $	10.200	&	230.586	$ \pm $	11.314	&	\ldots	&		&	99.39	&	134.1	\\
G 102--4 B	&		&	M4.0 V	&	D	&	RAO 552	&		\ldots		&		\ldots		&	\ldots	&		&	99.46	&	134.2	\\
\noalign{\smallskip}        \noalign{\smallskip}																									
V538 Aur	&		&	K1 V	&	A	&		&	81.499	$ \pm $	0.025	&	523.485	$ \pm $	0.032	&	0.16	&	Ros21	&		&		\\
HD 233153	&	J05415+534	&	M1.0 V	&	B	&	ENG 22	&	81.464	$ \pm $	0.023	&	515.975	$ \pm $	0.027	&	--0.02	&	Marf21	&	98.03	&	71.2	\\
\noalign{\smallskip}        \noalign{\smallskip}																									
HD 43587	&		&	G0 V	&	AB	&	CAT 1	&	51.616	$ \pm $	0.124	&	269.293	$ \pm $	0.196	&	--0.03	&	Mon18	&	0.84	&	70.9	\\
GJ 231.1 B	&	J06171+051	&	M3.5 V	&	CD	&	PRV 3	&	52.139	$ \pm $	0.083	&	261.646	$ \pm $	0.107	&	0.06	&	Kuz19	&	307.40	&	103.2	\\
\noalign{\smallskip}        \noalign{\smallskip}																									
HD 263175	&		&	K3 V	&	A	&		&	38.828	$ \pm $	0.022	&	467.065	$ \pm $	0.027	&	--0.24	&	Hir21	&		&		\\
HD 263175 B	&	J06461+325	&	M1.0 V	&	B	&	LDS 6201	&	38.873	$ \pm $	0.017	&	472.874	$ \pm $	0.025	&	\ldots	&		&	30.85	&	100.1	\\
\noalign{\smallskip}        \noalign{\smallskip}																									
HD 50281	&		&	K3.5 V	&	A	&		&	114.355	$ \pm $	0.042	&	543.702	$ \pm $	0.039	&	0.02	&	Ros21	&		&		\\
HD 50281 B	&	J06523--051	&	M2.0 V	&	B	&	WNO 17	&	114.291	$ \pm $	0.022	&	576.479	$ \pm $	0.031	&	0.10	&	Ros21	&	58.83	&	180.6	\\
\noalign{\smallskip}        \noalign{\smallskip}																									
GJ 3415	&		&	K4.5 V	&	A	&		&	39.870	$ \pm $	0.023	&	452.029	$ \pm $	0.026	&	\ldots	&		&		&		\\
GJ 3416	&	J06564+400	&	M0.5 V	&	B	&	KUI 27	&	39.925	$ \pm $	0.021	&	446.754	$ \pm $	0.026	&	--0.21	&	Gai14b	&	37.81	&	6.8	\\
\noalign{\smallskip}        \noalign{\smallskip}																									
V869 Mon	&		&	K3 V	&	A	&		&	71.032	$ \pm $	0.024	&	286.810	$ \pm $	0.030	&	0.03	&	Ros21	&		&		\\
HD 61606 B	&		&	K7 V	&	B	&	BGH 3	&	70.992	$ \pm $	0.025	&	294.206	$ \pm $	0.031	&	--0.11	&	Mon18	&	57.90	&	112.7	\\
GJ 282 C	&	J07361--031	&	M1.0 V	&	Cab	&	Pov09	&	70.275	$ \pm $	0.131	&	302.347	$ \pm $	0.173	&	--0.04	&	Marf21	&	296.71	&	3894.2	\\
\noalign{\smallskip}        \noalign{\smallskip}																									
HD 68146	&		&	F6.5 V	&	A	&		&	44.340	$ \pm $	0.053	&	257.608	$ \pm $	0.057	&	0.04	&	Luc18	&		&		\\
L 818--40 A	&	J08105--138	&	M2.5 V	&	B	&	LDS 204	&	44.520	$ \pm $	0.049	&	259.911	$ \pm $	0.058	&	\ldots	&		&	96.93	&	236.2	\\
L 818--40 B	&		&	M4.0 V	&	C	&	JOD 4	&	44.150	$ \pm $	0.203	&	245.493	$ \pm $	0.316	&	\ldots	&		&	97.54	&	236.6	\\
\noalign{\smallskip}        \noalign{\smallskip}																									
$\rho^{01}$ Cnc	&		&	K0  IV-V	&	A	&		&	79.448	$ \pm $	0.043	&	538.903	$ \pm $	0.055	&	0.38	&	Ros21	&		&		\\
$\rho^{01}$ Cnc B	&	J08526+283	&	M4.5 V	&	B	&	LDS 6219	&	79.656	$ \pm $	0.047	&	539.752	$ \pm $	0.053	&	--0.10	&	Marf21	&	84.83	&	128.1	\\
\noalign{\smallskip}        \noalign{\smallskip}																									
V405 Hya	&		&	K2 V	&	A	&		&	36.512	$ \pm $	0.022	&	112.027	$ \pm $	0.026	&	0.07	&	Luc18	&		&		\\
1RXS J090406.8--155512	&	J09040--159	&	M2.5 V	&	B	&	Sma21	&	36.628	$ \pm $	0.021	&	113.771	$ \pm $	0.025	&	\ldots	&		&	220.02	&	82.9	\\
\noalign{\smallskip}        \noalign{\smallskip}																									
BD+22 2086 A	&		&	K5 V	&	A	&		&	29.405	$ \pm $	0.020	&	218.392	$ \pm $	0.025	&	\ldots	&		&		&		\\
BD+22 2086 B	&	J09231+223	&	M0.0 V	&	B	&	HDS 1348	&	29.444	$ \pm $	0.022	&	223.161	$ \pm $	0.024	&	--0.10	&	Gai14b	&	8.30	&	343.4	\\
\noalign{\smallskip}        \noalign{\smallskip}																									
DX Leo	&		&	G9 V	&	A	&		&	55.329	$ \pm $	0.021	&	287.217	$ \pm $	0.025	&	0.07	&	Hir21	&		&		\\
HD 82443 B	&	J09328+269	&	M5.5 V	&	B	&	LDS 3903	&	55.292	$ \pm $	0.071	&	284.171	$ \pm $	0.086	&	\ldots	&		&	65.56	&	64.4	\\
\noalign{\smallskip}        \noalign{\smallskip}																									
HD 82939	&		&	G5 V	&	A	&		&	25.740	$ \pm $	0.023	&	134.640	$ \pm $	0.024	&	--0.08	&	Boc18	&		&		\\
GJ 9303	&	J09362+375	&	M0.0 V	&	Bab	&	Mal14a / SKF 254	&	25.836	$ \pm $	0.023	&	134.335	$ \pm $	0.025	&	--0.06	&	Jon20	&	301.52	&	162.3	\\
\noalign{\smallskip}        \noalign{\smallskip}																									
GJ 397.1	&		&	K5 V	&	A	&	LDS 2314	&	57.010	$ \pm $	0.014	&	185.374	$ \pm $	0.018	&	\ldots	&		&	141.96	&	225.6	\\
GJ 397.1 B	&	J10315+570	&	M4.5 V	&	BC	&	RAO 252	&		\ldots		&	161.307	$ \pm $	11.314	&	--0.01	&	Ter15a	&	225.59	&	142.0	\\
\noalign{\smallskip}        \noalign{\smallskip}																									
LZ UMa	&		&	G5 V	&	A	&		&	37.386	$ \pm $	0.070	&	196.647	$ \pm $	0.166	&	--0.11	&	Mon18	&		&		\\
GJ 3628	&	J10506+517	&	M3.5 V	&	B	&	LDS 3019	&	37.889	$ \pm $	0.028	&	191.404	$ \pm $	0.033	&	0.04	&	Ter15a	&	178.25	&	186.2	\\
\noalign{\smallskip}        \noalign{\smallskip}																									
HD 97584	&		&	K4 V	&	A	&		&	69.136	$ \pm $	0.015	&	418.802	$ \pm $	0.024	&	--0.17	&	Ston20	&		&	102.9	\\
HD 97584 B	&	J11151+734	&	M2.5 V	&	B	&	STF 1516	&	69.134	$ \pm $	0.018	&	396.508	$ \pm $	0.029	&	0.09	&	Gai14b	&	67.60	&	327.1	\\
\noalign{\smallskip}        \noalign{\smallskip}																									
GJ 426.1 A	&		&	F1 IV	&	Aab	&	Abt76	&	42.355	$ \pm $	0.398	&	169.810	$ \pm $	0.990	&	\ldots	&		&		&		\\
GJ 426.1 B	&		&	F5 V	&	B	&	STF 1536	&	41.496	$ \pm $	0.351	&	185.015	$ \pm $	0.974	&	\ldots	&		&	2.05	&	95.1	\\
LSPM J1123+1037	&	J11238+106	&	M0.5 V	&	C	&	STF 1536	&	41.667	$ \pm $	0.274	&	173.499	$ \pm $	0.303	&	\ldots	&		&	332.10	&	345.9	\\
\noalign{\smallskip}        \noalign{\smallskip}																									
HD 108421 A	&		&	K2 V	&	A	&		&	36.504	$ \pm $	0.027	&	265.137	$ \pm $	0.030	&	\ldots	&		&		&		\\
HD 108421 B	&		&	K4 V	&	B	&	STF 1643	&	36.511	$ \pm $	0.031	&	256.189	$ \pm $	0.037	&	\ldots	&		&	2.76	&	4.1	\\
CX Com	&	J12269+270	&	M4.5 V	&	C	&	LEP 54	&	37.636	$ \pm $	0.283	&	265.949	$ \pm $	0.405	&	0.00	&	Raj18a	&	221.40	&	260.9	\\
\noalign{\smallskip}        \noalign{\smallskip}																									
HD 115404	&		&	K2 V	&	A	&		&	91.018	$ \pm $	0.024	&	689.139	$ \pm $	0.042	&	--0.11	&	Ros21	&		&		\\
HD 115404 B	&	J13168+170	&	M0.5 V	&	B	&	BU 800	&	90.948	$ \pm $	0.023	&	701.233	$ \pm $	0.040	&	--0.28	&	Jon20	&	7.67	&	104.6	\\
\noalign{\smallskip}        \noalign{\smallskip}																									
GJ 9453	&		&	K5 V	&	A	&		&	25.386	$ \pm $	0.026	&	439.091	$ \pm $	0.046	&	\ldots	&		&		&		\\
GJ 9453 B	&	J13348+745	&	M3.5 V	&	B	&	LDS 1775	&	25.492	$ \pm $	0.015	&	437.055	$ \pm $	0.026	&	\ldots	&		&	14.80	&	323.3	\\
\noalign{\smallskip}        \noalign{\smallskip}																									
BD+21 2602	&		&	K4 V	&	A	&		&	24.815	$ \pm $	0.015	&	127.647	$ \pm $	0.019	&	\ldots	&		&		&		\\
StKM 1--1119	&	J14041+207	&	M1.0 V	&	B	&	J 1128	&		\ldots		&	132.085	$ \pm $	3.759	&	--0.20	&	Gai14b	&	62.66	&	190.2	\\
G3 1247168140942467200	&		&	M1.5 V	&	C	&	J 1128	&		\ldots		&		\ldots		&	\ldots	&		&	62.31	&	190.3	\\
\noalign{\smallskip}        \noalign{\smallskip}																									
HD 126660	&		&	F7 V	&	A	&		&	69.069	$ \pm $	0.158	&	464.153	$ \pm $	0.232	&	0.03	&	Luc17	&		&		\\
HD 126660 B	&	J14251+518	&	M2.5 V	&	B	&	STT 580	&	68.812	$ \pm $	0.032	&	469.652	$ \pm $	0.047	&	--0.14	&	Marf21	&	70.16	&	182.5	\\
\noalign{\smallskip}        \noalign{\smallskip}																									
KX Lib	&		&	K4 V	&	A	&		&	169.884	$ \pm $	0.065	&	2008.680	$ \pm $	0.087	&	--0.12	&	Mon18	&		&		\\
HD 131976	&	J14574--214	&	M1.5 V	&	BC	&	Mar87 / HN 28	&	168.770	$ \pm $	21.540	&	1933.943	$ \pm $	26.196	&	0.08	&	Mal20	&	306.60	&	25.8	\\
GJ 570 D	&		&	T8	&	D	&	BUG 4	&	169.300	$ \pm $	1.700	&	1972.880	$ \pm $	5.620	&	0.09	&	Bur13	&	234.00	&	317.0	\\
\noalign{\smallskip}        \noalign{\smallskip}																									
HD 135363	&		&	G5 V	&	AB	&	MET 10	&	33.711	$ \pm $	0.052	&	208.703	$ \pm $	0.102	&	--0.07	&	Gui09	&	0.36	&	133.1	\\
LSPM J1507+7613	&	J15079+762	&	M4.5 V	&	C	&	LEP 72	&	33.714	$ \pm $	0.027	&	207.105	$ \pm $	0.058	&	\ldots	&		&	116.45	&	1.7	\\
\noalign{\smallskip}        \noalign{\smallskip}																									
HD 144579	&		&	G8 V	&	A	&		&	69.641	$ \pm $	0.014	&	573.293	$ \pm $	0.023	&	--0.53	&	Ros21	&		&		\\
HD 144579 B	&	J16048+391	&	M4.0 V	&	B	&	WNO 47	&	69.637	$ \pm $	0.019	&	564.436	$ \pm $	0.030	&	--0.62	&	Ter15a	&	70.00	&	280.1	\\
\noalign{\smallskip}        \noalign{\smallskip}																									
$\sigma$ CrB A	&		&	F6 V	&	Aab	&	Str03 / Rag09	&	44.057	$ \pm $	0.046	&	282.061	$ \pm $	0.072	&	--0.01	&	Luc17	&		&		\\
$\sigma$ CrB B	&		&	G1 V	&	B	&	STF 2032	&	44.134	$ \pm $	0.018	&	301.273	$ \pm $	0.026	&	--0.02	&	Ros21	&	7.23	&	238.5	\\
$\sigma$ CrB C	&	J16139+337	&	M2.5 V	&	CD	&	STF 2032	&	44.267	$ \pm $	0.159	&	300.693	$ \pm $	0.241	&	\ldots	&		&	241.15	&	635.1	\\
\noalign{\smallskip}        \noalign{\smallskip}																									
V1090 Her	&		&	K3 V	&	A	&		&	55.751	$ \pm $	0.016	&	308.703	$ \pm $	0.031	&	0.01	&	Ros21	&		&		\\
HD 153557 B	&	J16578+473	&	M1.5 V	&	B	&	A 1874	&	55.771	$ \pm $	0.017	&	301.441	$ \pm $	0.033	&	--0.43	&	Pas18	&	5.09	&	63.0	\\
V1089 Her	&		&	K3 V	&	C	&	STFA 32	&	55.718	$ \pm $	0.016	&	296.941	$ \pm $	0.028	&	--0.03	&	Ros21	&	112.38	&	261.6	\\
\noalign{\smallskip}        \noalign{\smallskip}																									
HD 154363	&		&	K4.5 V	&	A	&		&	95.567	$ \pm $	0.024	&	1461.664	$ \pm $	0.032	&	--0.23	&	Ros21	&		&		\\
HD 154363 B	&	J17052--050	&	M1.5 V	&	B	&	LDS 585	&	95.560	$ \pm $	0.021	&	1457.065	$ \pm $	0.028	&	--0.39	&	Marf21	&	184.42	&	122.7	\\
\noalign{\smallskip}        \noalign{\smallskip}																									
HD 160269 A	&		&	G0 IV/V	&	AB	&	BU 962	&	69.283	$ \pm $	0.200	&	522.563	$ \pm $	0.334	&	--0.04	&	Tau20	&	0.63	&	300.5	\\
GJ 685	&	J17355+616	&	M0.5 V	&	C	&	LDS 2736	&	69.892	$ \pm $	0.015	&	577.333	$ \pm $	0.023	&	--0.03	&	Marf21	&	738.16	&	160.3	\\
\noalign{\smallskip}        \noalign{\smallskip}																									
HD 161797	&		&	G5 IV	&	AB	&	TRN 2	&	119.925	$ \pm $	0.154	&	833.789	$ \pm $	0.217	&	0.32	&	Ros21	&	1.78	&	254.8	\\
GJ 695 B	&		&	M2.5 V	&	C	&	STF 2220	&	119.887	$ \pm $	0.206	&	899.446	$ \pm $	0.279	&		&		&	35.36	&	248.9	\\
GJ 695 C	&	J17464+277	&	M3.5 V	&	D	&	AC 7	&	120.398	$ \pm $	0.279	&	719.401	$ \pm $	0.489	&		&		&	0.58	&	335.9	\\
\noalign{\smallskip}        \noalign{\smallskip}																									
BD+31 3330	&		&	K2.5 V	&	A	&		&	41.745	$ \pm $	0.016	&	841.174	$ \pm $	0.024	&	--0.31	&	Hir21	&		&		\\
BD+31 3330 B	&	J18409+315	&	M1.0 V	&	B	&	HJ 1337	&		\ldots		&		\ldots		&	\ldots	&		&	9.45	&	152.2	\\
BD+31 3330 C	&		&	M1.0 V	&	C	&		&		\ldots		&		\ldots		&	\ldots	&		&	9.21	&	153.1	\\
\noalign{\smallskip}        \noalign{\smallskip}																									
HD 187691	&		&	F8 V	&	A	&		&	51.313	$ \pm $	0.090	&	277.688	$ \pm $	0.108	&	0.15	&	Hir21	&		&		\\
GJ 9671 B	&	J19510+104	&	M3.5 V	&	B	&	J 124	&	51.373	$ \pm $	0.040	&	288.376	$ \pm $	0.052	&	\ldots	&		&	21.48	&	220.2	\\
\noalign{\smallskip}        \noalign{\smallskip}																									
HD 190360	&		&	G7 IV-V	&	A	&		&	62.487	$ \pm $	0.035	&	861.921	$ \pm $	0.045	&	0.23	&	Ros21	&		&		\\
GJ 777 B	&	J20034+298	&	M4.5 V	&	B	&	LDS 6339	&	62.527	$ \pm $	0.022	&	860.495	$ \pm $	0.030	&		&		&	178.05	&	232.3	\\
\noalign{\smallskip}        \noalign{\smallskip}																									
HD 191785	&		&	K0 V	&	A	&		&	48.926	$ \pm $	0.023	&	575.386	$ \pm $	0.025	&	--0.04	&	Ros21	&		&		\\
GJ 783.2 B	&	J20112+161	&	M4.0 V	&	B	&	GIC 163	&	48.928	$ \pm $	0.032	&	577.775	$ \pm $	0.038	&	--0.04	&	Kuz19	&	103.84	&	94.8	\\
\noalign{\smallskip}        \noalign{\smallskip}																									
StKM 1--1767a	&		&	K5 V	&	A	&		&	27.359	$ \pm $	0.018	&	108.284	$ \pm $	0.023	&	\ldots	&		&		&		\\
{[}R78b{]} 440	&	J20132+029	&	M1.0 V	&	B	&	CRI 26	&	27.359	$ \pm $	0.023	&	110.727	$ \pm $	0.029	&	0.36	&	Gai14b	&	32.50	&	123.9	\\
\noalign{\smallskip}        \noalign{\smallskip}																									
HD 197076	&		&	G5 V	&	A	&	LDS 1045	&	47.746	$ \pm $	0.020	&	334.027	$ \pm $	0.023	&	--0.07	&	Ros21	&		&		\\
GJ 797 B	&	J20407+199	&	M2.5 V	&	BC	&	RAO  23	&		\ldots		&	339.095	$ \pm $	1.980	&	--0.07	&	Pas18	&	184.06	&	125.1	\\
\noalign{\smallskip}        \noalign{\smallskip}																									
GJ 9728 B	&		&	G5 V	&	AB	&	AGC 13	&	49.576	$ \pm $	0.463	&	472.404	$ \pm $	1.069	&	\ldots	&		&	1.05	&	189.7	\\
GJ 822.1 C	&	J21147+380	&	M2.5 V	&	CD	&	AGC 13	&	49.105	$ \pm $	0.042	&	453.205	$ \pm $	0.059	&	--0.08	&	Gai14b	&	184.45	&	89.9	\\
\noalign{\smallskip}        \noalign{\smallskip}																									
V447 Lac	&		&	K1 V	&	A	&		&	45.591	$ \pm $	0.017	&	223.871	$ \pm $	0.023	&	0.09	&	Hir21	&		&		\\
GJ 4269	&	J22160+546	&	M4.0 V	&	B	&	GIC 177	&	45.625	$ \pm $	0.020	&	221.350	$ \pm $	0.032	&	--0.04	&	Man15	&	76.90	&	107.4	\\
\noalign{\smallskip}        \noalign{\smallskip}																									
HD 216385	&		&	F6 V	&	A	&	LDS 6388	&	36.558	$ \pm $	0.108	&	523.347	$ \pm $	0.197	&	--0.11	&	Stei20	&	249.64	&	19.6	\\
GJ 9801 B	&	J22524+099	&	M3.0 V	&	BC	&	RAO 30	&	37.250	$ \pm $	0.760	&	530.182	$ \pm $	11.314	&	\ldots	&		&	250.25	&	19.6	\\
\noalign{\smallskip}        \noalign{\smallskip}																									
V368 Cep	&		&	G9 V	&	A	&		&	52.784	$ \pm $	0.014	&	215.918	$ \pm $	0.022	&	--0.03	&	Man15	&		&		\\
HD 220140 B	&	J23194+790	&	M3.5 V	&	B	&	LDS 2035	&	52.840	$ \pm $	0.021	&	218.080	$ \pm $	0.036	&	\ldots	&		&	10.91	&	214.1	\\
LP 12--90	&	J23228+787	&	M5.0 V	&	C	&	MKR 1	&	52.834	$ \pm $	0.030	&	217.441	$ \pm $	0.051	&	\ldots	&		&	962.74	&	141.1	\\
\noalign{\smallskip}        \noalign{\smallskip}																									
StKM 2--1787	&		&	K4 V	&	A	&		&	26.840	$ \pm $	0.020	&	120.688	$ \pm $	0.026	&	--0.49	&	Mon18	&		&		\\
PM J23535+1206S	&	J23535+121	&	M2.5 V	&	B	&	VYS  11	&	26.792	$ \pm $	0.035	&	119.437	$ \pm $	0.045	&	--0.06	&	Gai14b	&	5.78	&	165.1	\\
\noalign{\smallskip}        \noalign{\smallskip}																																									
\end{longtable}
\tablefoot{
\tablefoottext{a}{References for discovery --
Kat13: \cite{Kat13};
Mal14a: \cite{Mal14a};
Mar87: \cite{Mar87};
Pov09: \cite{Pov09};
Rag09: \cite{Rag09};
Ros21: \cite{Ros21};
She85: \cite{She85};
Sma21: \cite{Sma21};
Str03: \cite{Str03};
Tor09: \cite{Tor09};
Zak79: \cite{Zak79}.
}
\tablefoottext{b}{References for metallicities --
Boc18: \cite{Boc18};
Bud21: \cite{Bud21};
Bur13: \cite{Bur13};
Gai14b: \cite{Gai14b};
Gui09: \cite{Gui09};
Hir21: \cite{Hir21};
Hou16: \cite{Hou16};
Jon20: \cite{Jon20};
Kuz19: \cite{Kuz19};
Luc17: \cite{Luc17};
Luc18: \cite{Luc18};
Man15: \cite{Man15};
Mal20: \cite{Mal20};
Man15: \cite{Man15};
Marf21: \cite{Marf21};
Mas08: \cite{Mas08};
Mon18: \cite{Mon18};
Pas18: \cite{Pas18};
Raj18a: \cite{Raj18a};
Ric20: \cite{Ric20};
Ros21: \cite{Ros21};
Stei20: \cite{Stei20};
Ston20: \cite{Ston20};
Tau20: \cite{Tau20};
Ter15a: \cite{Ter15a};
Tin19: \cite{Tin19};
Zak22: \cite{Zak22}.}
}
\end{landscape}
}


==> tables/table_SB.tex <==
{\fontsize{8}{10}\selectfont 
\begin{longtable}{llccccl}
\caption{Spectroscopic binaries, triples, and quadruples in our sample.}
\label{tab:spectroscopic}
\\

    \hline\hline 
    \noalign{\smallskip}
    Name	&	Karmn	&	Type$^a$	&	$P_{\rm orb}$ [d]			&	$a \sin{i}$ [au]	&	$q = \mathcal{M}_B/\mathcal{M}_A$&	Reference$^b$	\\
    \noalign{\smallskip}
    \hline
    \noalign{\smallskip}
\endfirsthead
\caption{Spectroscopic binaries, triples, and quadruples in our sample (cont.).}\\
    \hline\hline 
    Name	&	Karmn	&	Type$^a$	&	$P_{\rm orb}$ [d]			& $a \sin{i}$ [au]	&	$q = \mathcal{M}_B/\mathcal{M}_A$&	Reference$^b$	\\
    \noalign{\smallskip}
    \hline
    \noalign{\smallskip}
\endhead
%
\hline
\endfoot
%
HD 38A	&		&	SB	&		\ldots		&	\ldots	&	\ldots	&	Abt70, Str93	\\
1RXS J000806.3+475659	&	J00081+479	&	SB2	&	<4.4			&	0.04	&	\ldots	&	Shk10, Fou18	\\
EZ Psc	&	J00162+198W	&	SB2	&	3.95652	 $\pm$ 	0.00008	&	0.038623	&	0.35	&	Bar18	\\
FF And	&	J00428+355	&	SB2	&		\ldots		&	\ldots	&	\ldots	&	Bop77, Giz02	\\
RX J0050.2+0837	&	J00502+086	&	SB2	&		\ldots		&	\ldots	&	\ldots	&	Jef18	\\
GJ 1029	&	J01056+284	&	SB2	&	95.76	 $\pm$ 	0.18	&	0.1331	&	0.72	&	Bar18, Win20	\\
PM J01437--0602	&	J01437--060	&	SB2	&		\ldots		&	\ldots	&	\ldots	&	Fou18	\\
G 173--18	&	J01453+465	&	SB2	&	<157.9			&	0.56	&	\ldots	&	Giz02, Shk10	\\
BD--21 332	&	J01531--210	&	SB2	&	<2.9			&	0.04	&	\ldots	&	Shk10	\\
GJ 1041 B	&	J01592+035W	&	SB2	&	<356.4			&	0.93	&	\ldots	&	Shk10	\\
GJ 3129	&	J02027+135	&	SB2	&	<27.8			&	0.13	&	\ldots	&	Jen09, Shk10	\\
GJ 3131	&	J02033--212	&	SB2	&		\ldots		&	\ldots	&	\ldots	&	Jef18	\\
V374 And	&	J02069+451	&	SB2	&	897.0	 $\pm$ 	2.3	&	\ldots	&	0.70	&	Spe19	\\
GJ 3160	&	J02289+120	&	SB2	&		\ldots		&	\ldots	&	\ldots	&	Jef18	\\
GJ 3235	&	J03346--048	&	ST3	&		\ldots		&	\ldots	&	\ldots	&	Jef18	\\
GJ 3236	&	J03372+691	&	DESB2	&	0.7712600	 $\pm$ 	0.0000023	&	0.0143	&	0.75	&	Irw09, Shk10	\\
GJ 3239	&	J03375+178N	&	SB2	&	<33.2			&	0.18	&	\ldots	&	Shk10, Fou18	\\
GJ 3240	&	J03375+178S	&	SB2	&	<0.4			&	0.01	&	\ldots	&	Shk10	\\
HD 278874	&		&	SB2	&		\ldots		&	\ldots	&	\ldots	&	Mon18	\\
Wolf 227	&	J03526+170	&	SB2	&		\ldots		&	\ldots	&	\ldots	&	Bon13a, Jef18	\\
HD 24916 B	&	J03574--011	&	SB	&		\ldots		&	\ldots	&	\ldots	&	Zak79	\\
LP 414--117	&	J04123+162	&	SB2	&	128.114			&	\ldots	&	0.60	&	Ben08	\\
1RXS J042441.9--064725	&	J04247--067	&	ST3	&	<1.9			&	0.02	&	\ldots	&	Shk10	\\
GJ 3282	&	J04252+080S	&	SB2	&		\ldots		&	\ldots	&	\ldots	&	Jef18	\\
LP 775--31	&	J04352--161	&	SB2	&		\ldots		&	\ldots	&	\ldots	&	Rei09	\\
TYC 694--1183--1	&	J04414+132	&	SB	&		\ldots		&	\ldots	&	\ldots	&	Mer09	\\
LP 415--345	&	J04425+204	&	SB2	&		\ldots		&	\ldots	&	\ldots	&	Sta97	\\
LP 416--43	&	J04480+170	&	SB	&	8.49474	 $\pm$ 	0.00007	&	6.2	&	\ldots	&	Gri85	\\
1RXS J044847.6+100302	&	J04488+100	&	SB2	&		\ldots		&	\ldots	&	\ldots	&	Jef18	\\
GJ 3322 A	&	J05019+099	&	SB2	&		\ldots		&	\ldots	&	0.57	&	Del98, Del99b	\\
HD 285190	&	J05032+213	&	SB2	&		\ldots		&	\ldots	&	\ldots	&	Jef18, Fou18	\\
Capella	&		&	SB2	&	104.02173	 $\pm$ 	0.00022	&	0.7357	&	0.99	&	She85, Tor09	\\
GJ 1080	&	J05282+029	&	SB	&		\ldots		&	\ldots	&	\ldots	&	Jen09	\\
HD 35956	&		&	SB1	&		\ldots		&	\ldots	&	\ldots	&	Kat13	\\
Ross 42	&	J05322+098	&	SB2	&	<61.1			&	0.23	&	1.00	&	Mar87, Shk10	\\
V371 Ori	&	J05337+019	&	SB1	&	0.60417356	 $\pm$ 	0.00000025	&	\ldots	&	\ldots	&	Rein12, Bar21	\\
Ross 45 B	&	J05342+103S	&	SB	&		\ldots		&	\ldots	&	\ldots	&	Rein12	\\
V1402 Ori	&	J05402+126	&	SB2	&	<138.9			&	0.52	&	\ldots	&	Shk10	\\
Wolf 237	&	J05466+441	&	SB2	&		\ldots		&	\ldots	&	\ldots	&	Jef18	\\
Ross 59	&	J05532+242	&	SB2	&	721	 $\pm$ 	2	&	0.6656	&	0.33	&	Bar18	\\
LP 86--173	&	J06054+608	&	SB1	&	0.30992678	 $\pm$ 	0.00000048	&	0.0049	&	0.93	&	New16, Win20	\\
TYC 4525--194--1	&	J06171+751	&	ST3?	&		\ldots		&	\ldots	&	\ldots	&	Fou18	\\
G 108--4	&	J06298--027	&	SB2	&	<46.9			&	0.16	&	\ldots	&	Shk10	\\
1RXS J070005.1--190115	&	J07001--190	&	SB2	&	6.56025	 $\pm$ 	0.00030	&	0.002797	&	\ldots	&	Bar21	\\
QY Aur	&	J07100+385	&	SB2	&	10.42673	 $\pm$ 	0.00010	&	0.0687	&	0.85	&	TP86, Win20	\\
TYC 4530--1414--1	&	J07119+773	&	SB1	&		\ldots		&	\ldots	&	\ldots	&	Jef18	\\
1RXS J073138.4+455718	&		&	SB2?	&		\ldots		&	\ldots	&	\ldots	&	Fou18	\\
GJ 3447	&	J07320+173E	&	SB	&		\ldots		&	\ldots	&	\ldots	&	Gaia22a	\\
Castor	&		&	SB2 + SB2	&	167570	 $\pm$ 	840	&	83.9052	&	0.79	&	Bel97, Cur06, Tor22	\\
Castor C	&	J07346+318	&	DESB2	&	0.8142822	 $\pm$ 	0.0000010	&	0.01809	&	1.00	&	Joy26, Giz02, Tor02, Tor22	\\
GJ 282 C	&	J07361--031	&	SB1	&	6591	 $\pm$ 	177	&	6.224	&	0.34	&	Bar21	\\
GJ 3461	&	J07418+050	&	EB?/SB2	&		\ldots		&	\ldots	&	\ldots	&	Jef18	\\
1RXS J075434.3+083213	&	J07545+085	&	SB1	&		\ldots		&	\ldots	&	\ldots	&	Jef18	\\
FP Cnc B	&	J08089+328	&	SB2	&	<395.5			&	0.92	&	\ldots	&	Shk10	\\
CU Cnc	&	J08316+193S	&	DESB2	&	2.771468	 $\pm$ 	0.000004	&	0.03624	&	0.92	&	Del99a, Del99b, Tor10	\\
LSPM J0835+1408	&	J08353+141	&	ST3	&		\ldots		&	\ldots	&	\ldots	&	Ski18	\\
GJ 319 A	&	J08427+095	&	SB1	&	20.9491	 $\pm$ 	0.0019	&	0.021	&	0.22	&	Duq88	\\
GJ 3522	&	J08589+084	&	SB2	&	7.5555	 $\pm$ 	0.0002	&	\ldots	&	0.82	&	Rei97b, Del99b	\\
GJ 3540	&	J09120+279	&	SB2	&		\ldots		&	\ldots	&	\ldots	&	Jef18	\\
LP 427--16	&	J09140+196	&	SB1	&		\ldots		&	\ldots	&	\ldots	&	Bar21	\\
HD 79210	&	J09143+526	&	SB1	&		\ldots		&	\ldots	&	\ldots	&	Jef18	\\
GJ 9303	&	J09362+375	&	SB2	&		\ldots		&	\ldots	&	\ldots	&	Mal14a	\\
LP 728--70	&	J09506--138	&	SB2	&		\ldots		&	\ldots	&	\ldots	&	Jef18	\\
GJ 372	&	J09531--036	&	SB2	&	47.709	 $\pm$ 	0.053	&	39.06	&	0.76	&	Har96, Jef18, Bar18	\\
GJ 373	&	J09561+627	&	SB?	&		\ldots		&	\ldots	&	\ldots	&	Rein12	\\
LP 790--2	&	J10182--204	&	SB2	&	5.922845	 $\pm$ 	0.000061	&	0.048242	&	0.58	&	Bar18	\\
GJ 3612	&	J10354+694	&	SB2	&	119.41	 $\pm$ 	0.04	&	0.3464	&	0.51	&	Bar18	\\
LP 127--502	&	J10368+509	&	SB2?	&		\ldots		&	\ldots	&	\ldots	&	Fou18	\\
GJ 3626	&	J10504+331	&	SB1	&	2996	 $\pm$ 	31	&	0.2355	&	\ldots	&	Bar21	\\
GJ 3630	&	J10520+005	&	ST3/SQ4	&	<28.1			&	0.11	&	\ldots	&	Shk10	\\
LP 491--51	&	J11036+136	&	SB1	&		\ldots		&	\ldots	&	\ldots	&	Jef18	\\
GJ 426.1 A	&		&	SB	&		\ldots		&	\ldots	&	\ldots	&	Abt76	\\
GJ 455	&	J12023+285	&	SB2	&		\ldots		&	\ldots	&	\ldots	&	Giz02	\\
LP 734--34	&	J12104--131	&	SB2	&	33.6551	 $\pm$ 	0.0046	&	0.0479	&	0.95	&	Win20	\\
GJ 3719	&	J12169+311	&	SB2	&		\ldots		&	\ldots	&	\ldots	&	Fou18	\\
G 148--43	&	J12191+318	&	SB2	&		\ldots		&	\ldots	&	\ldots	&	Jef18	\\
GJ 3731	&	J12299--054W	&	SB2	&		\ldots		&	\ldots	&	\ldots	&	Jef18	\\
G 123--45	&	J12364+352	&	SB1	&	34.7557	 $\pm$ 	0.0041	&	0.0219	&	\ldots	&	Win20	\\
DP Dra	&	J12490+661	&	ST3	&	54.075	 $\pm$ 	0.006	&	\ldots	&	0.95	&	Del99b	\\
GJ 507 B	&	J13195+351E	&	SB1	&		\ldots		&	\ldots	&	\ldots	&	Jef18	\\
GQ Vir	&	J14130--120	&	SB2	&		\ldots		&	\ldots	&	\ldots	&	Jef18	\\
GJ 1182	&	J14155+046	&	SB2	&	154.2	 $\pm$ 	0.1	&	0.35835	&	0.66	&	Bar18	\\
PM J14171+0851	&	J14171+088	&	SB2	&		\ldots		&	\ldots	&	\ldots	&	Jef18	\\
GJ 3861	&	J14368+583	&	SB2	&		\ldots		&	\ldots	&	\ldots	&	Giz02, Jef18	\\
GJ 3875	&	J14549+411	&	SB	&		\ldots		&	\ldots	&	\ldots	&	Ski18	\\
G 136--35	&	J14564+168	&	SB	&		\ldots		&	\ldots	&	\ldots	&	Ski18	\\
StKM 1--1240	&	J15238+561	&	SB2	&		\ldots		&	\ldots	&	\ldots	&	Fou18	\\
GJ 3910	&	J15319+288	&	SB1	&		\ldots		&	\ldots	&	\ldots	&	Jen09	\\
UU UMi	&	J15412+759	&	SB2	&	5240	 $\pm$ 	410	&	4.7	&	0.59	&	Bar18, Bar21	\\
GJ 595	&	J15421--194	&	SB1	&		\ldots		&	\ldots	&	\ldots	&	Nid02	\\
GJ 3916	&	J15474--108	&	ST3	&	3028	 $\pm$ 	23	&	3.59	&	1.05	&	Bar21	\\
LP 177--102	&	J15474+451	&	DESB2	&	3.5500184	 $\pm$ 	0.0000018	&	0.036535	&	1.00	&	Moc02, Har11, Bir12	\\
$\sigma$ CrB A	&		&	SB2	&	1.139791423	 $\pm$ 	0.00000008	&	0.013106	&	0.96	&	Str03, Rag09	\\
CM Dra	&	J16343+571	&	DESB2	&	1.268389985	 $\pm$ 	0.000000005	&	0.017502	&	0.93	&	Mor09, Tor10, Scha19	\\
V1054 Oph	&	J16554--083S	&	ST3	&	2.965522	 $\pm$ 	0.000014	&	0.05	&	0.90	&	Joy47, Pet84, Del98	\\
LP 331--57 A	&	J17038+321	&	SB2?	&		\ldots		&	\ldots	&	\ldots	&	Shk09, Fou18	\\
GJ 3991	&	J17095+436	&	SB1	&		\ldots		&	\ldots	&	\ldots	&	Rei97b, Del99b	\\
Wolf 1473	&	J17464--087	&	SB2	&	83.926	 $\pm$ 	0.032	&	0.27559	&	0.93	&	Mal14a, Win20	\\
GJ 1230 A	&	J18411+247S	&	SB2	&	5.0688	 $\pm$ 	0.00005	&	\ldots	&	0.95	&	GR96, Del99b  	\\
GJ 735	&	J18554+084	&	SB2	&		\ldots		&	\ldots	&	\ldots	&	Mar87, Giz02, Kar04	\\
GJ 4091 B	&	J18563+544	&	SB2	&		\ldots		&	\ldots	&	\ldots	&	Fou18	\\
G 125--15	&	J19312+361	&	SB2	&	<0.7			&	0.01	&	\ldots	&	Shk10	\\
RX J1935.4+3746	&	J19354+377	&	SB1	&		\ldots		&	\ldots	&	\ldots	&	Shk09, Jef18	\\
LP 869--19	&	J19420--210	&	SB2	&		\ldots		&	\ldots	&	\ldots	&	Mal14a	\\
{V1513 Cyg} & {J20050+544} & {SB1} & {0.49670418 $\pm$ 0.00000005} & {0.010537 $\pm$ 0.000005} & \ldots & {Giz97b, Mac18} \\
LP 574--21	&	J20105+065	&	SB2	&	<40.1			&	0.19	&	\ldots	&	Shk10	\\
LP 395--8 A	&	J20198+229	&	SB2	&	1.1293392	 $\pm$ 	0.0000067	&	0.01057	&	0.56	&	Bar18	\\
1RXS J203011.0+795040	&	J20301+798	&	SB2	&		\ldots		&	190.469	&	\ldots	&	Jef18	\\
GJ 4155	&	J20409--101	&	SB	&		\ldots		&	\ldots	&	\ldots	&	Rei12	\\
GJ 4161	&	J20445+089N	&	SB2	&		\ldots		&	\ldots	&	\ldots	&	Jef18	\\
GJ 810 A	&	J20556--140N	&	SB2	&	812	 $\pm$ 	51	&	0.841	&	0.83	&	Bar18	\\
FR Aqr	&	J20568--048	&	SB2	&		\ldots		&	\ldots	&	\ldots	&	Jef18	\\
Ross 775	&	J21296+176	&	SB2	&	53.221	 $\pm$ 	0.004	&	\ldots	&	1.00	&	Mar87, Del99b	\\
GJ 4213	&	J21442+066	&	SB1	&		\ldots		&	\ldots	&	\ldots	&	Jef18	\\
EZ Aqr	&	J22385--152	&	ST3	&	822.6	 $\pm$ 	0.6	&	1189	&	0.53	&	Del99c	\\
FK Aqr	&	J22387--206S	&	SB2	&	4.08322	 $\pm$ 	0.00004	&	0.039372	&	0.80	&	Her65, Del99b	\\
FL Aqr	&	J22387--206N	&	SB1	&	1.795	 $\pm$ 	0.017	&	0.00353	&	0.60	&	Dav14	\\
LP 521--79	&	J23063+126	&	SB2(3?)	&	<58.9			&	0.31	&	\ldots	&	Shk10	\\
GJ 4314	&	J23096--019	&	SB2	&		\ldots		&	\ldots	&	\ldots	&	Jef18	\\
GJ 4327	&	J23174+382	&	SB2	&		\ldots		&	\ldots	&	\ldots	&	Jef18	\\
GJ 1284	&	J23302--203	&	SB2	&	11.838033	 $\pm$ 	0.000076	&	6.48275	&	0.19	&	Giz02, Jef18, Car21	\\
Ross 676	&	J23439+647	&	SB2	&	<3			&	0.04	&	\ldots	&	Shk10	\\
GJ 912	&	J23556--061	&	SB1	&	5188	 $\pm$ 	58	&	0.505	&	0.12	&	Bar21	\\
GJ 4379	&	J23573--129W	&	SB2	&		\ldots		&	\ldots	&	\ldots	&	Giz02, Jef18	\\
Wolf 1051	&	J23585+076	&	ST3	&	4634	 $\pm$ 	17	&	0.4436	&	0.55	&	Bar21	\\
\noalign{\smallskip}
\hline
\end{longtable}
\tablefoot{
\tablefoottext{a}{ 
A spectroscopic binary (SB) that displays one or two lines in the spectrum is a single- or double-lined spectroscopic binary, respectively, and abbreviated as SB1 or SB2.
A spectroscopic triple (ST) showing two or three lines is a double- or triple-lined spectroscopic triple, and abbreviated as ST2 or ST3.
Spectroscopic quadruples (SQ) are much more rare, and typically are three- or four-lined systems, denominated SQ3 and SQ4, respectively. 
In our sample, only one star is classified as SQ4 (\object{GJ~3630}, J10520+005).
}
\tablefoottext{b}{While recognising the contributions of contemporary investigations 
(e.g. \citealt{Shk10}, \citealt{Jef18}, \citealt{Bar18,Bar21}, and \citealt{Win20} are the source of many of the parameters in this table), references are often limited for simplicity to the original sources that first identified the systems. 
However, exceptions are made for prominent systems such as \object{Castor~C} or nearby stars with a long history of observations, such as \object{CM~Dra} and \object{CU~Cnc}. References --
Abt70: \cite{Abt70};
Bar18: \cite{Bar18};
Bar21: \cite{Bar21};
Bel97: \cite{Bel97};
Ben08: \cite{Ben08};
Bir12: \cite{Bir12};
Bon13a: \cite{Bon13a};
Bop77: \cite{Bop77};
Cur06: \cite{Cur06};
Dav14: \cite{Dav14};
Del98: \cite{Del98};
Del99a: \cite{Del99a};
Del99b: \cite{Del99b};
Del99c: \cite{Del99c};
Fou18: \cite{Fou18};
Gaia22a: \cite{Gaia22a};
Giz02: \cite{Giz02};
{Giz97b: \cite{Giz97b};}
GR96: \cite{GR96};
Har11: \cite{Har11};
Har96: \cite{Har96};
Her65: \cite{Her65};
Irw09: \cite{Irw09};
Jef18: \cite{Jef18};
Jen09: \cite{Jen09};
Joy26: \cite{Joy26};
Joy47: \cite{Joy47};
Kar04: \cite{Kar04};
Kat13: \cite{Kat13};
Mac02: \cite{Moc02};
{Mac18: \cite{Mac18};}
Mal14a: \cite{Mal14a};
Mar87: \cite{Mar87};
Mer09: \cite{Mer09};
Moc02: \cite{Moc02};
Mon18: \cite{Mon18};
Mor09: \cite{Mor09};
New16: \cite{New16};
Nid02: \cite{Nid02};
Pet84: \cite{Pet84};
Rag09: \cite{Rag09};
Rei09: \cite{Rei09};
Rein12: \cite{Rein12};
Rei97b: \cite{Rei97b};
Scha19: \cite{Scha19};
She85: \cite{She85};
Shk09: \cite{Shk09};
Shk10: \cite{Shk10};
Shk12: \cite{Shk12};
Ski18: \cite{Ski18};
Spe19: \cite{Spe19};
Sta97: \cite{Sta97};
Ste14: \cite{Ste14};
Str03: \cite{Str03};
Str93: \cite{Str93};
TP86: \cite{TP86};
Tor09: \cite{Tor09};
Tor22: \cite{Tor22};
Win20: \cite{Win20};
Zak79: \cite{Zak79}.
}
}
}

==> tables/table_UCD.tex <==
\begin{longtable}{lllllcccc}
\caption{\label{tab:ucd} Multiple systems containing M dwarfs and ultra-cool dwarfs.}
\\
\noalign{\smallskip}
\noalign{\smallskip}
\hline
\hline
\noalign{\smallskip}
Name	&	Karmn	&	Spectral	&	Comp.	&	Discoverer$^b$	&	$\pi$			&	$\mu_{\rm total}$			&	$\rho$	&	$\theta$	\\
	&		&	type$^a$	&		&		&	{[}mas{]}			&	{[}mas\,a$^{-1}${]}			&	{[}arcsec{]}	&	{[}deg{]}	\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
\endfirsthead
\caption{Multiple systems containing M dwarfs and ultra-cool dwarfs (continued).}\\
\hline\hline
        \noalign{\smallskip}
Name	&	Karmn	&	Spectral	&	Comp.	&	Discoverer$^b$	&	$\pi$			&	$\mu_{\rm total}$			&	$\rho$	&	$\theta$	\\
	&		&	type$^a$	&		&		&	{[}mas{]}			&	{[}mas\,a$^{-1}${]}			&	{[}arcsec{]}	&	{[}deg{]}	\\
\hline
\noalign{\smallskip}
\endhead
%
\hline
\endfoot
\noalign{\smallskip}
GJ 3131	&	J02033--212	&	M2.5 V	&	Aab	&	Jef18	&	46.672	$ \pm $	0.041	&	471.895	$ \pm $	0.051	&	\ldots	&	\ldots	\\
GJ 3131 B	&		&	L0:	&	B	&	Sma21	&	46.747	$ \pm $	0.307	&	450.045	$ \pm $	0.474	&	4.008	&	252.0	\\
\noalign{\smallskip}        \noalign{\smallskip}																					
G 196--3	&	J10043+503	&	M2.5 V	&	A	&		&	45.854	$ \pm $	0.019	&	246.664	$ \pm $	0.022	&		&		\\
G 196--3 B	&		&	L3$\beta$	&	B	&	REB 1	&	46.195	$ \pm $	0.545	&	246.291	$ \pm $	0.673	&	16.070	&	209.2	\\
\noalign{\smallskip}        \noalign{\smallskip}																					
GJ 3657	&	J11231+258	&	M5.0 V	&	A	&		&	61.652	$ \pm $	0.064	&	1061.305	$ \pm $	0.100	&		&		\\
2M J11225550+2550250	&		&	T6	&	B	&	WIS 183	&	62.9	$ \pm $	2.8	&	1062.3	$ \pm $	4.6	&	254.985	&	221.300	\\
\noalign{\smallskip}        \noalign{\smallskip}																					
Wolf 462	&	J13007+123	&	M1.5 V	&	AB	&	BEU 16	&	86.901	$ \pm $	0.117	&	629.606	$ \pm $	0.227	&	0.525	&	60.0	\\
Ross 458 C	&		&	T8.5p	&	C	&	GDM 1	&	85.540	$ \pm $	1.530	&	639.451	$ \pm $	13.454	&	12.060	&	220.2	\\
\noalign{\smallskip}        \noalign{\smallskip}																					
LP 738--14	&	J13481--137	&	M4.5 V	&	A	&		&	55.028	$ \pm $	0.024	&	858.148	$ \pm $	0.037	&		&		\\
LP 738--14 B	&		&	T5.5	&	B	&	DEA 1	&	59.500	$ \pm $	3.600	&	857.920	$ \pm $	5.371	&	67.340	&	291.50	\\
\noalign{\smallskip}        \noalign{\smallskip}																					
GJ 9492	&	J14423+660	&	M2.0 V	&	A	&		&	91.479	$ \pm $	0.016	&	301.514	$ \pm $	0.028	&		&		\\
GJ 9492 B	&		&	L0	&	B	&	GKI 4	&	91.357	$ \pm $	0.091	&	337.307	$ \pm $	0.177	&	2.290	&	93.6	\\
\noalign{\smallskip}        \noalign{\smallskip}																					
KX Lib	&		&	K4 V	&	A	&		&	169.884	$ \pm $	0.065	&	2008.680	$ \pm $	0.087	&		&		\\
HD 131976	&	J14574--214	&	M1.5 V	&	BC	&	Mar87, HN 28	&	168.770	$ \pm $	21.540	&	1933.943	$ \pm $	26.196	&	25.762	&	306.6	\\
GJ 570 D	&		&	T8	&	D	&	BUG 4	&	169.300	$ \pm $	1.700	&	1972.880	$ \pm $	5.620	&	234.0	&	317.0	\\
\noalign{\smallskip}        \noalign{\smallskip}																					
GJ 618.1 A	&	J16204--042	&	M0.0 V	&	A	&		&	34.076	$ \pm $	0.019	&	416.694	$ \pm $	0.032	&		&		\\
GJ 618.1 B	&		&	L2.5	&	B	&	WIL 3	&	33.872	$ \pm $	0.759	&	415.281	$ \pm $	1.118	&	35.907	&	144.8	\\
\noalign{\smallskip}        \noalign{\smallskip}																					
G 259--20	&	J17431+854	&	M2.0 V	&	A	&		&	45.255	$ \pm $	0.314	&	291.245	$ \pm $	0.527	&		&		\\
2M J17430860+8526594	&		&	L5	&	B	&	LUH 12	&	45.139	$ \pm $	0.280	&	290.996	$ \pm $	0.501	&	29.739	&	358.4	\\
\noalign{\smallskip}        \noalign{\smallskip}																					
GJ 4040	&	J17578+465	&	M2.5 V	&	A	&		&	71.495	$ \pm $	0.015	&	578.336	$ \pm $	0.028	&		&		\\
G 204--39 B	&		&	T7	&	B	&	BDK 9	&	73.750	$ \pm $	1.840	&	594.569	$ \pm $	21.932	&	197.0	&	130.6	\\
\noalign{\smallskip}        \noalign{\smallskip}																					
V1513 Cyg	&	J20050+544	&	M1.0 V	&	A	&		&	60.296	$ \pm $	0.027	&	1470.281	$ \pm $	0.050	&		&		\\
Wolf 1130 B	&		&	T8p	&	B	&	MGN 1	&		\ldots		&		\ldots		&	188.5	&	115.00	\\
\noalign{\smallskip}        \noalign{\smallskip}																					
LP 395--8 A	&	J20198+229	&	M3.0 V	&	Aab	&	Bar18	&	33.897	$ \pm $	0.026	&	135.400	$ \pm $	0.027	&	\ldots	&	\ldots	\\
LP 395--8 B	&		&	M3.5: V	&	B	&	KPP 4191	&	33.896	$ \pm $	0.053	&	137.726	$ \pm $	0.057	&	1.918	&	355.5	\\
G3 1829571684884360832	&		&	L2:	&	C	&	This work	&	33.938	$ \pm $	0.342	&	142.755	$ \pm $	0.359	&	11.019	&	307.4	\\
\noalign{\smallskip}        \noalign{\smallskip}																					
G 126--32 A	&		&	M1.0: V	&	A	&		&	27.661	$ \pm $	0.127	&	219.436	$ \pm $	0.143	&		&		\\
G 126--32 B	&	J21450+198	&	M1.5 V	&	B	&	RAO 466	&	26.818	$ \pm $	0.296	&	240.736	$ \pm $	0.412	&	0.564	&	253.3	\\
G 126--32 C	&		&	L1	&	C	&	Sma21	&	26.252	$ \pm $	0.803	&	232.177	$ \pm $	1.024	&	5.317	&	16.4	\\
\noalign{\smallskip}        \noalign{\smallskip}																					
Wolf 940	&	J21466--001	&	M4.0 V	&	A	&		&	80.738	$ \pm $	0.052	&	920.673	$ \pm $	0.060	&		&		\\
Wolf 940 B	&		&	T8	&	B	&	BNG 2	&	79.800	$ \pm $	4.500	&	919.0			&	31.640	&	250.5	\\
\noalign{\smallskip}        \noalign{\smallskip}																					
Wolf 1154 A	&	J22012+323	&	M1.5 V	&	A	&		&	32.344	$ \pm $	0.024	&	133.621	$ \pm $	0.029	&		&		\\
Wolf 1154 B	&		&	M3.5: V	&	B	&	GRV 1283	&	32.418	$ \pm $	0.083	&	119.082	$ \pm $	0.085	&	1.302	&	235.5	\\
2M J22011701+3222062	&		&	T2.5	&	C	&		&	31.400	$ \pm $	5.400	&	125.765	$ \pm $	2.702	&	80.750	&	147.6	\\
\noalign{\smallskip}        \noalign{\smallskip}																					
GJ 4287	&	J22374+395	&	M0.0 V	&	AB	&	HDS 3211	&	46.887	$ \pm $	0.564	&	365.030	$ \pm $	0.836	&	0.261	&	11.0	\\
G 216--7 B	&		&	M9.5 V	&	C	&	KIR 5	&	47.644	$ \pm $	0.137	&	351.145	$ \pm $	0.206	&	33.332	&	111.5	\\
\noalign{\smallskip}        \noalign{\smallskip}														
\end{longtable}
\tablefoot{
\tablefoottext{a}{When spectroscopic classification is not available, a semicolon (:) denotes an estimated spectral type from absolute magnitude $M_G$.}
\tablefoottext{b}{References:
Jef18: \cite{Jef18};
Mar87: \cite{Mar87};
Bar18: \cite{Bar18};
Sma21: \cite{Sma21}.
Other alphanumeric correspond to the WDS discoverer code. 
}
}



==> tables/table_WD.tex <==
{\fontsize{7}{10}\selectfont 
\begin{longtable}{llllcccccccc}
\caption{\label{tab:wd} Multiple systems containing M dwarfs and white dwarfs.}
\\
\noalign{\smallskip}
\noalign{\smallskip}
\noalign{\smallskip}
\hline
\hline
\noalign{\smallskip}
Name	&	Karmn	&	Spectral	&	Discoverer$^b$	&	$\pi$			&	$\mu_{\rm total}$			&	$\rho^c$	&	$\theta$	\\
	&		&	type$^a$	&		&	{[}mas{]}			&	{[}mas\,a$^{-1}${]}			&	{[}arcsec{]}	&	{[}deg{]}	\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
\endfirsthead
\caption{Multiple systems containing M dwarfs and white dwarfs (cont.).}\\
\hline\hline
        \noalign{\smallskip}
Name	&	Karmn	&	Spectral	&	Discoverer$^b$	&	$\pi$			&	$\mu_{\rm total}$			&	$\rho^c$	&	$\theta$	\\
	&		&	type$^a$	&		&	{[}mas{]}			&	{[}mas\,a$^{-1}${]}			&	{[}arcsec{]}	&	{[}deg{]}	\\
\hline
\noalign{\smallskip}
\endhead
%
\hline
\endfoot
GJ 1015 B	&		&	DBQ5	&		&	43.659	$ \pm $	0.022	&	324.163	$ \pm $	0.025	&		&		\\
GJ 1015 A	&	J00413+558	&	M4.0 V	&	GIC  13	&	43.735	$ \pm $	0.022	&	332.499	$ \pm $	0.024	&	10.854	&	248.4	\\
\noalign{\smallskip}        \noalign{\smallskip}																			
GJ 3118	&		&	DA5.6	&		&	57.799	$ \pm $	0.016	&	301.944	$ \pm $	0.018	&		&		\\
GJ 3117	&	J01518+644	&	M2.5 V	&	GIC  27	&	57.825	$ \pm $	0.016	&	306.369	$ \pm $	0.018	&	13.503	&	0.7	\\
\noalign{\smallskip}        \noalign{\smallskip}																			
GJ 3151$^d$	&	J02204+377	&	M2.5 V + DA	&	LDS 3370	&	40.867	$ \pm $	0.033	&	349.298	$ \pm $	0.050	&	2.0	&	89.0	\\
\noalign{\smallskip}        \noalign{\smallskip}																			
LSPM J0401+5131	&		&	DC8	&		&	39.836	$ \pm $	0.077	&	883.245	$ \pm $	0.117	&		&		\\
Ross 25	&	J04011+513	&	M3.5 V	&	Sma21	&	39.816	$ \pm $	0.021	&	883.463	$ \pm $	0.028	&	494.0	&	173.4	\\
\noalign{\smallskip}        \noalign{\smallskip}																			
o$^{02}$ Eri B	&		&	DA2.9	&		&	199.691	$ \pm $	0.051	&	4018.591	$ \pm $	0.061	&		&		\\
o$^{02}$ Eri	&		&	K0 V	&	STF 518	&	199.608	$ \pm $	0.121	&	4089.836	$ \pm $	0.165	&	83.337	&	282.2	\\
o$^{02}$ Eri C	&	J04153--076	&	M4.5 V	&	STF 518	&	199.452	$ \pm $	0.069	&	4083.715	$ \pm $	0.084	&	78.097	&	277.5	\\
\noalign{\smallskip}        \noalign{\smallskip}																			
GJ 169.1 B	&		&	DC5	&		&	181.273	$ \pm $	0.020	&	2361.129	$ \pm $	0.028	&		&		\\
GJ 169.1 A	&	J04311+589	&	M4.0 V	&	STI 2051	&	181.244	$ \pm $	0.050	&	2424.355	$ \pm $	0.073	&	10.263	&	238.2	\\
\noalign{\smallskip}        \noalign{\smallskip}																			
GJ 3431	&		&	DQ8	&		&	41.029	$ \pm $	0.036	&	357.871	$ \pm $	0.053	&		&		\\
GJ 3430	&	J07102+376	&	M4.0 V	&	GIC  69	&	44.601	$ \pm $	0.437	&	350.218	$ \pm $	0.608	&	12.472	&	223.1	\\
\noalign{\smallskip}        \noalign{\smallskip}																			
G 107--70 A	&		&	DA	&		&	83.484			&	1281.725	$ \pm $	3.606	&		&		\\
G 107--70 B	&		&	DA	&	GIC  75	&		\ldots		&		\ldots		&	0.667	&	318.1	\\
GJ 275.2 A$^e$	&	J07307+481	&	M4.0 V	&	WNO 49	&	88.723	$ \pm $	0.030	&	1287.988	$ \pm $	0.034	&	103.1	&	333.9	\\
\noalign{\smallskip}        \noalign{\smallskip}																			
GJ 283 A	&		&	DZQA6	&		&	109.344	$ \pm $	0.018	&	1261.341	$ \pm $	0.024	&		&		\\
GJ 283 B	&	J07403--174	&	M6.0 V	&	LUY 5693	&	109.254	$ \pm $	0.039	&	1270.984	$ \pm $	0.052	&	20.338	&	279.5	\\
\noalign{\smallskip}        \noalign{\smallskip}																			
GJ 401 B	&		&	DQ	&		&	53.190	$ \pm $	0.034	&	1962.558	$ \pm $	0.057	&		&		\\
GJ 401	&	J10456--191	&	M0.5 V	&	LDS 4013	&	53.172	$ \pm $	0.022	&	1963.772	$ \pm $	0.034	&	6.655	&	174.5	\\
\noalign{\smallskip}        \noalign{\smallskip}																			
GJ 1142 B	&		&	DA3	&		&	40.293	$ \pm $	0.032	&	446.106	$ \pm $	0.042	&		&		\\
GJ 1142 A	&	J11081--052	&	M3.0 V	&	LDS 852	&	40.180	$ \pm $	0.026	&	443.166	$ \pm $	0.034	&	279.0	&	159.3	\\
\noalign{\smallskip}        \noalign{\smallskip}																			
GJ 1155 B	&		&	DA	&		&	42.773	$ \pm $	0.043	&	711.074	$ \pm $	0.064	&		&		\\
GJ 1155 A	&	J12168+029	&	M3.0 V	&	LDS 935	&	42.820	$ \pm $	0.035	&	700.554	$ \pm $	0.054	&	2.126	&	357.9	\\
\noalign{\smallskip}        \noalign{\smallskip}																			
Wolf 485	&		&	DA3.5	&		&	62.148	$ \pm $	0.044	&	1207.505	$ \pm $	0.056	&		&		\\
Ross 476	&	J13300--087	&	M4.0 V	&	LDS 448	&	62.281	$ \pm $	0.042	&	1210.608	$ \pm $	0.059	&	502.4	&	198.7	\\
\noalign{\smallskip}        \noalign{\smallskip}																			
GJ 1179 B	&		&	DC9	&		&	84.311	$ \pm $	0.029	&	1490.906	$ \pm $	0.041	&		&		\\
GJ 1179 A	&	J13482+236	&	M5.5 V	&	LDS 4410	&	84.225	$ \pm $	0.027	&	1487.630	$ \pm $	0.037	&	188.1	&	49.5	\\
\noalign{\smallskip}        \noalign{\smallskip}																			
GJ 630.1 B	&		&	DQ8	&	LDS 1436	&	67.354	$ \pm $	0.021	&	1634.847	$ \pm $	0.035	&		&		\\
CM Dra	&	J16343+571	&	M4.5 V	&	Mor09, Tor10	&	67.288	$ \pm $	0.034	&	1623.346	$ \pm $	0.061	&	26.726	&	201.9	\\
\noalign{\smallskip}        \noalign{\smallskip}																			
LP 387--36	&		&	DC7	&		&	28.841	$ \pm $	0.054	&	285.375	$ \pm $	0.072	&		&		\\
LP 387--37	&	J17058+260	&	M1.5 V	&	LDS 4721	&	28.746	$ \pm $	0.019	&	291.032	$ \pm $	0.025	&	19.244	&	179.6	\\
\noalign{\smallskip}        \noalign{\smallskip}																			
LSPM J1826+1120S	&		&	DA	&		&	37.055	$ \pm $	0.066	&	281.066	$ \pm $	0.092	&		&		\\
GJ 4059	&	J18264+113	&	M3.5 V	&	NI   38	&	37.056	$ \pm $	0.024	&	276.066	$ \pm $	0.033	&	8.196	&	16.8	\\
\noalign{\smallskip}        \noalign{\smallskip}																			
LP 141--14	&		&	DC	&		&	40.393	$ \pm $	0.051	&	246.401	$ \pm $	0.095	&		&		\\
G 229--20 A	&	J18576+535	&	M3.5 V	&	LDS 4802	&	40.348	$ \pm $	0.015	&	261.445	$ \pm $	0.028	&	43.653	&	343.9	\\
LP 141--13	&		&	M3.0 V	&	LDS 4802	&	40.365	$ \pm $	0.015	&	245.563	$ \pm $	0.027	&	2.290	&	17.0	\\
\noalign{\smallskip}        \noalign{\smallskip}																			
GJ 754.1 A	&		&	DBQA5	&		&	95.176	$ \pm $	0.029	&	173.039	$ \pm $	0.038	&		&		\\
GJ 754.1 B	&	J19205--076	&	M2.5 V	&	LDS 678	&	95.178	$ \pm $	0.031	&	191.462	$ \pm $	0.037	&	27.168	&	306.2	\\
\noalign{\smallskip}        \noalign{\smallskip}																			
V1513 Cyg$^f$	&		&	sdM1.5 + WD 	&	Giz97b	&	60.296	$ \pm $	0.027	&	1470.281	$ \pm $	0.050	&	0.010537 {[}au{]}	&		\\
Wolf 1130 C	&	J20050+544	&	T8p	&	MGN1	&	62.9	$ \pm $	3.3	&		\ldots		&	188.54	&	115.00	\\
\noalign{\smallskip}        \noalign{\smallskip}																			
V1412 Aql	&		&	DC7	&		&	43.574	$ \pm $	0.038	&	635.705	$ \pm $	0.051	&		&		\\
GJ 784.2 A	&	J20139+066	&	M3.5 V	&	GIC 164	&	43.570	$ \pm $	0.022	&	634.751	$ \pm $	0.029	&	101.5	&	150.9	\\
\noalign{\smallskip}        \noalign{\smallskip}																			
Ross 193 B	&		&	DC10	&	LDS 6420	&	61.760	$ \pm $	0.052	&	807.720	$ \pm $	0.068	&		&		\\
FR Aqr	&	J20568--048	&	M4.0 V	&	Jef18	&	61.824	$ \pm $	0.074	&	826.321	$ \pm $	0.091	&	15.006	&	129.4	\\
\noalign{\smallskip}        \noalign{\smallskip}																			
UCAC4 747--070768	&		&	DAH	&		&	118.155	$ \pm $	0.016	&	88.850	$ \pm $	0.026	&		&		\\
TYC 3980--1081--1	&	J21516+592	&	M4.0 V	&	KPP 4252	&	123.057	$ \pm $	0.594	&	79.885	$ \pm $	1.668	&	14.642	&	291.9	\\
\noalign{\smallskip}        \noalign{\smallskip}																			
Gaia DR3 2005884249925303168$^g$	&		&	D?	&		&	18.550	$ \pm $	0.079	&	108.971	$ \pm $	0.123	&		&		\\
LF 4 +54 152	&	J22129+550	&	M0.0 V	&	Sma21	&	18.385	$ \pm $	0.153	&	109.131	$ \pm $	0.248	&	66.265	&	209.8	\\
\noalign{\smallskip}        \noalign{\smallskip}																			
GJ 4305	&		&	DA8.1	&		&	40.325	$ \pm $	0.072	&	439.472	$ \pm $	0.074	&		&		\\
GJ 4304	&	J22559+057	&	M1.0 V	&	LDS 5021	&	40.347	$ \pm $	0.024	&	446.045	$ \pm $	0.029	&	17.168	&	104.6	\\
\noalign{\smallskip}        \noalign{\smallskip}																			
LSPM J2309+5506E	&		&	DA	&		&	60.895	$ \pm $	0.030	&	410.185	$ \pm $	0.039	&		&		\\
G 233--42	&	J23089+551	&	M5.0 V	&	NSN  11	&	60.921	$ \pm $	0.027	&	411.267	$ \pm $	0.035	&	6.150	&	249.6	\\
\noalign{\smallskip}        \noalign{\smallskip}																			
GJ 4357	&		&	DA	&		&	25.367	$ \pm $	0.100	&	325.253	$ \pm $	0.126	&		&		\\
GJ 4356	&	J23389+210	&	M3.5 V	&	LDS 5108	&	25.402	$ \pm $	0.028	&	328.855	$ \pm $	0.036	&	9.495	&	290.7	\\
\noalign{\smallskip}        \noalign{\smallskip}																			
GJ 905.2 B	&		&	DA3.8	&	LDS 1070	&	53.762	$ \pm $	0.027	&	224.052	$ \pm $	0.039	&	174.7	&	10.0	\\
GJ 905.2 A	&	J23438+325	&	M3.0 V	&	JOD 26	&		\ldots		&	223.766	$ \pm $	13.688	&	0.109	&	128.0	\\
\noalign{\smallskip}        \noalign{\smallskip}																													
\end{longtable}
\tablefoot{
\tablefoottext{a}{In Simbad's taxonomy of white dwarfs, `D’ stands for degenerate, followed by an abbreviation of the most significant spectral features: 
`A’ for a hydrogen-rich atmosphere,
`B’ for a helium-rich atmosphere,
`C’ for no strong spectral lines,
`Q’ for carbon lines, and
`Z’ for metal lines.}
\tablefoottext{b}{References —
Mor09: \cite{Mor09};
Tor10: \cite{Tor10};
Jef18: \cite{Jef18};
Sma21: \cite{Sma21}.}
\tablefoottext{c}{{Angular separation $\rho$ and position angle $\theta$ measured from the white dwarf.}}
\tablefoottext{d}{GJ~3151: White dwarf in a compact configuration ($s \simeq 49$\,au) determined spectroscopically \citep{Schi12} but not resolved by {\em Gaia}.}
\tablefoottext{e}{\object{GJ~275.2~A}: it has a closer companion according to \cite{Har81}, who determined a 0.94-year period and individual masses of 0.17 and 0.08\,$\mathcal{M}_\odot$.
They also estimated a mean angular separation of $\sim$ 0.05\,arcsec, which is compatible with the application of Third Kepler's law.}
\tablefoottext{f}{{\object{Wolf~1130} is a 0.4967-day binary composed of a subdwarf (sdM1.5; \citealt{Giz97b}) and a white dwarf, likely bound to evolve into a cataclysmic variable \citep{Mac18}.}}
\tablefoottext{g}{Gaia~DR3 2005884249925303168:
Unconfirmed spectroscopically but proposed candidate to WD in agreement with \cite{Jim18} based on position in HR diagram.
}
}
}


==> tables/table_description.tex <==
{\fontsize{8}{10}\selectfont 
\begin{longtable}{lccl}
\caption{\label{tab:description} Description of the online table.}
\\
    \hline
    \hline 
    \noalign{\smallskip}
    Parameter & Units & Column(s) & Description \\
    \noalign{\smallskip}
    \hline
    \noalign{\smallskip}
\endfirsthead
%
\caption{Description of the online table (cont.).}\\
\hline\hline
\noalign{\smallskip}
    Parameter & Units & Column(s) & Description \\
\hline
\noalign{\smallskip}
\endhead
%
\hline
\endfoot
%
\multicolumn{4}{l}{\em Identification} \\		\hline			
{\tt ID\_star, ID\_system}	&	\ldots	&	1, 2	&	Star and system identifiers$^a$	\\
{\tt Name}	&	\ldots	&	3	&	Discovery name or most common name$^b$	\\
{\tt GJ}	&	\ldots	&	4	&	Gliese-Jahreiss catalogue number$^c$	\\
{\tt Karmn}	&	\ldots	&	5	&	Carmencita star identifier (JHHMMm+DDd)$^d$	\\
{\tt RA\_J2016, DE\_J2016}	&	hms, dms	&	6, 7	&	Right ascension and declination in the epoch J2016.0	\\
{\tt SpT, SpTnum, SpT\_ref}	&	\ldots	&	8--10	&	Spectral type, its numerical format, and the reference$^e$	\\
\hline		\multicolumn{4}{l}{\em Multiplicity} \\		\hline			
{\tt Type, Class}	&	\ldots	&	11, 12	&	Type of system and multiplicity class$^f$	\\
{\tt Component, System}	&	\ldots	&	13, 14	&	Component designation and their resolution$^g$	\\
{\tt SB, SB\_ref}	&	\ldots	&	15, 16	&	Type of spectroscopic system and reference$^h$	\\
{\tt Discoverer}	&	\ldots	&	17	&	Discoverer code$^i$	\\
{\tt Group, Group\_ref}	&	\ldots	&	18, 19	&	Stellar group (SKG, cluster or association) and reference$^j$	\\
{\tt Nplanet, Planet\_ref}	&	\ldots	&	20, 21	&	Number of confirmed planets and reference	\\
{\tt Category}	&	\ldots	&	22	&	Category 1--3 as described in Sect.~\ref{ssection:fraction}	\\
{\tt Remarks}	&	\ldots	&	23	&	Comments and remarks on multiplicity	\\
{\tt WDS\_...}	&	\ldots	&	24--32	&	Washington double star catalogue data$^k$	\\
{\tt s01, s02}	&	au	&	33, 37	&	Physical separation between the components in multiple systems$^l$	\\
{\tt s01\_ref}	&	\ldots	&	36	&	Reference for the closest component$^m$	\\
{\tt rho01, rho02}	&	arcsec	&	34, 38	&	Projected angular separation ($s = \rho d$)	\\
{\tt theta01, theta02}	&	deg	&	35, 39	&	Positional angle$^n$	\\
{\tt muratio, deltaPA, deltad}	&	\ldots	&	40--42	&	$\mu{\rm ratio}$, $\Delta PA$, $\Delta d$ criteria for physical association$^o$	\\
\hline		\multicolumn{4}{l}{\em Stellar parameters} \\		\hline			
{\tt M\_Msol, eM\_Msol}	&	$\mathcal{M}_\odot$	&	43, 44	&	Stellar mass and its error 	\\
{\tt R\_Rsol, eR\_Msol}	&	$\mathcal{R}_\odot$	&	45, 46	&	Stellar radius and its error 	\\
{\tt MR\_ref}	&	\ldots	&	47	&	Reference for mass and radius	\\
{\tt L\_Lsol, eL\_Lsol, L\_ref}	&	$\mathcal{L}_\odot$	&	48--50	&	Luminosity, error, and reference	\\
{\tt MG\_mag, eMG\_mag}	&	mag	&	51, 52	&	Absolute magnitude in $G$ and its error	\\
{\tt Teff\_K, eTeff\_K, Teff\_K\_ref}	&	K	&	53--55	&	Effective temperature and its error	\\
{\tt logg, elogg}	&	dex	&	56, 57	&	Surface gravity and its error (reference shared with {\tt L\_Lsol})	\\
{\tt Fe\_H, Fe\_H\_ref }	&	\ldots	&	58, 59	&	Iron abundance (metallicity) and its error	\\
\hline		\multicolumn{4}{l}{\em System parameters} \\		\hline			
{\tt q}	&	\ldots	&	60	&	Mass ratio	\\
{\tt P01, eP01, P01\_ref, P02, eP02}	&	d, a	&	61--65	&	Orbital periods, errors and reference	\\
{\tt Ug\_J, eUg\_J}	&	J	&	66, 67	&	Binding energy and its error	\\
{\tt crit\_...}	&	Boolean	&	68--75	&	Criteria for unresolved companions$^p$	\\
{\tt Candidate}	&	Boolean	&	76	&	Candidate to unresolved companion$^q$	\\
\hline		\multicolumn{4}{l}{\em Astrometry} \\		\hline			
{\tt \_id}	&	\ldots	&	77--79	&	Catalogue identifiers	\\
{\tt ra, ra\_error}	&	deg	&	80, 81	&	Barycentric right ascension and its error in the epoch {J2016.0}	\\
{\tt dec, dec\_error}	&	deg	&	82, 83	&	Barycentric declination and its error in the epoch {J2016.0} 	\\
{\tt parallax, parallax\_error, parallax\_ref}	&	mas	&	84--86	&	Parallax, error and reference	\\
{\tt pmra, pmra\_error, pmdec, pmdec\_error, pm\_ref}	&	mas\,a$^{-1}$	&	87--91	&	Proper motion in right ascension and declination, errors, and reference	\\
{\tt rv, rv\_error, rv\_ref}	&	km\,s$^{-1}$	&	92--94	&	Radial velocity, error, and reference	\\
{\tt ruwe}	&	\ldots	&	95	&	Renormalised unit weight error from {\em Gaia} DR3	\\
{\tt {[}Statistics DR3{]}}	&	\ldots	&	96--110	&	Additional statistical indicators in {\em Gaia} DR3$^r$	\\
\hline		\multicolumn{4}{l}{\em Photometry} \\		\hline

{\tt NN\_mag, eNN\_mag, Qf\_MM}	&	mag	&	111--132	&	Photometric magnitudes and quality flags in up to 10 passbands$^s$	\\

\end{longtable}
\tablefoot{
\tablefoottext{a}{\texttt{ID\_star} is a unique identifier that sorts the table by right ascension but prioritising that components of the same system (equal \texttt{ID\_system}) are together and sorted by decreasing brightness.}\\
\tablefoottext{b}{Name of the star, Simbad-searchable, obeying the following priority ($n$ designates a natural number): 
Proper name,
variable in constellation (V* V$n$ Con; but not suspected variables, SV*),
Henry Draper (HD~$n$, with $n \leq$ 225300),
Gliese-Jahreiss (GJ~$n$, only if $n<$ 4000),
Bonner Durchmusterung (BD$\pm n$~$n$),
Luyten (LP~$n$-$n$),
Giclas (G~$n$-$n$, only if unique Giclas designation),
Luyten (LHS~$n$),
other designations in chronological order (Haro, StKM/StM, 1RXS/RXS, HIP, LSPM, PM, NLTT, GSC, TYC, MCC, R78b, I81, 2MUCD),
catalog identifier ({\em Gaia}~DR3, 2MASS, UCAC4).}\\
\tablefoottext{c}{Gliese-Jahreiss (GJ) designation entry, when available. This includes the first catalogue by \cite{Gli57} and its update \citep{Gli69}, the supplement by \cite{Woo70}, and the succeeding editions \citep{GJ79}.}\\
\tablefoottext{d}{``HHMMm$\pm$DDd'' are the truncated equatorial coordinates.
For close stars with separations less than 5\,arcsec, a position of the star in the system is added as ``N'', ``S'', ``E'' or ``W''.}\\
\tablefoottext{e}{{\tt SpTnum} = 10.0 for O0.0\,V, 20.0 for B0.0\,V, 30.0 for A0.0\,V, 40.0 for F0.0\,V, 50.0 for G0.0\,V, 60.0 for K0.0\,V, 70.0 for M0.0\,V, 70.5 for M0.5\,V, 80.0 for L0. The values 0.0 and 999 are reserved for white dwarfs and stars with a luminosity class other than main sequence (V), respectively.
Spectral types were rounded when necessary (e.g. M0.0 instead of M0.1, or M4.0 instead of M3.8).
`This work' refers to spectral type photometric estimation from absolute magnitudes as \cite{Cif20}.}\\
\tablefoottext{f}{`Candidate' and `Multiple+' must be read as `new unresolved binary candidate'.}\\
\tablefoottext{g}{The system nomenclature follows the scheme in Fig.~\ref{fig:nomenclature}.}\\
\tablefoottext{h}{Definitions of SB1, SB2, ST2, ST3, and SQ are shown in Table~\ref{tab:spectroscopic}.}\\
\tablefoottext{i}{WDS discoverer code or literature reference.}\\
\tablefoottext{j}{Abbreviations follow the scheme outlined in Table~\ref{tab:skg}.}\\
\tablefoottext{k}{{\tt id}: WDS identifier (see also column {\tt Discoverer}); 
{\tt comp}: Component designations;
{\tt obs1, obs2}: First and last observation years;
{\tt pa2}: Positional angle in the most recent measurement;
{\tt sep2}: Separation in the most recent measurement;
{\tt mag1, mag2}: Magnitudes of the two components.
More details can be found in the WDS website: \url{http://www.astro.gsu.edu/wds/}.}\\
\tablefoottext{l}{In systems of three or more components, {\tt 01} denotes the separation between the closest components, i.e., {\tt s01} $<$ {\tt s02}.}\\
\tablefoottext{m}{The reference is displayed when the value is not calculated in this work using {\em Gaia} data. The reference for {\tt s02} is {\em Gaia} in all cases. This also applies to the orbital periods.}\\
\tablefoottext{n}{Measured eastward from the north in the epoch 2016.0. In the programmatic computation of this parameter caution must be taken regarding the ``quadrant ambiguity'', i.e., a 180-deg erroneous difference.}\\
\tablefoottext{o}{For triple or higher-order systems, this association refers to the primary component.}\\
\tablefoottext{p}{Criteria for physical association ({\tt crit\_association}) and statistical metrics from {\em Gaia} as described in Table~\ref{tab:criteria} ({\tt crit\_ruwe, crit\_ipd\_ruwe, crit\_rv, crit\_rv\_error, crit\_ipd\_fmp, crit\_dupl\_source, crit\_non\_single, crit\_DR3\_non\_single}).
Orbital: Orbital model for an astrometric binary; OrbitalTargetedSearch: Orbital model for a priori known systems, with a subset containing suffix `Validated'; SB1: Single-lined spectroscopic binary; SB2: Double-lined spectroscopic binary; SB2C: Double-lined spectroscopic binary with circular orbit; AstroSpectroSB1: Combined astrometric and single lined spectroscopic orbital model.}\\
\tablefoottext{q}{It refers to unknown unresolved binaries. That is, if an unresolved companion already exists (e.g. an spectroscopic binary), the value is `false’ regardless of the {\em Gaia} metrics (Table~\ref{tab:criteria}).}\\
\tablefoottext{r}{Statistics from DR3 related to the criteria for unresolved binarity:
{\tt 
astrometric\_excess\_noise, 
astrometric\_excess\_noise\_sig, 
phot\_bp\_rp\_excess\_factor, 
phot\_bp\_n\_blended\_transits, 
phot\_rp\_n\_blended\_transits,
phot\_variable\_flag,
rv\_chisq\_pvalue, 
rv\_amplitude\_robust,
rv\_nb\_transits,  
renormalised\_gof,
astrometric\_n\_obs\_al, 
astrometric\_n\_good\_obs\_al,
ipd\_gof\_harmonic\_amplitude,
duplicated\_source
} (see Sect.~\ref{ssection:unresolved}).}\\
\tablefoottext{s}{
{\tt BP}, {\tt G}, {\tt RP}: $G_{B_P}$, $G$, and $G_{R_P}$ from {\em Gaia} DR3 \citep{Gaia23}; 
{\tt J}, {\tt H}, {\tt Ks}: $J$, $H$, and $Ks$ from 2MASS \citep{Skr06}; 
{\tt W1}, {\tt W2}, {\tt W3}, {\tt W4}: $W1$, $W2$, $W3$, and $W4$ from AllWISE \citep{Cut14}.
The photometric uncertainties in the {\em Gaia} passbands have been calculated by us $\Delta \lambda = |-2.5/ \ln{10} \times \Delta F_\lambda/F_\lambda|$, where $F_\lambda$ and $\Delta F_\lambda$ are the flux and its error in the $\lambda$ passband, using the errors in the corresponding fluxes, and the zero points as provided by VizieR.}\\
}}

==> tables/table_exoplanets.tex <==
\begin{longtable}{llllcl}
\caption{\label{tab:exoplanets} Stars hosting planets in our sample.}\\
\noalign{\smallskip}
\hline\hline
\noalign{\smallskip} 
Name	&	Karmn	&	Spectral	&	System	&	Number of	&	Discovery$^b$	\\
	&		&	type	&	class	&	planets$^a$	&	\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
\endfirsthead
\caption{Stars hosting planets in our sample (cont.).}\\
\hline\hline
\noalign{\smallskip}        
Name	&	Karmn	&	Spectral	&	System	&	Number of	&	Discovery$^b$	\\
	&		&	type	&	class	&	planets$^a$	&		\\
\hline
\noalign{\smallskip}
\endhead
%
\hline
\endfoot
GJ 1002	&	J00067--075	&	M5.5 V	&	Single	&	2	&	Sua23	\\
GJ 12	&	J00158+135	&	M3.0 V	&	Single	&	1	&	Kuz24, Dho24	\\
GX And	&	J00183+440	&	M1.0 V	&	Multiple	&	2	&	How14, Pin18	\\
TOI--1470	&	J00403+612	&	M2.0 V	&	Single	&	2	&	Gon23b	\\
GJ 3053	&	J00449--152	&	M4.5 V	&	Single	&	2	&	Dit17, Men19	\\
GJ 3072	&	J01023--104	&	M0.0 V	&	Single	&	1	&	Fen20	\\
Wolf 46	&	J01026+623	&	M1.5 V	&	Multiple	&	1	&	Per19	\\
LSPM J0106+1913	&	J01066+192	&	M3.0 V	&	Single	&	2	&	Cha22	\\
YZ Cet	&	J01125--169	&	M4.5 V	&	Single	&	2	&	Ast17b, Sto20a	\\
Ross 19	&	J02190+353	&	M3.5 V	&	Single	&	1	&	Sch21	\\
PM J02489--1432W	&	J02489--145W	&	M2.0 V	&	Multiple	&	1	&	Kos21	\\
Teegarden's Star	&	J02530+168	&	M7.0 V	&	Single	&	2	&	Zec19, Dre24	\\
HD 18143 A	&		&	K2 IV	&	Multiple	&	2	&	Fen22	\\
LP 14--53	&	J02573+765	&	M4.0 V	&	Single	&	1	&	Sot21	\\
GJ 3193	&	J03018--165S	&	M3.5 V	&	Multiple	&	2	&	Win19b, Win22	\\
CD Cet	&	J03133+047	&	M5.0 V	&	Single	&	1	&	Bau20	\\
o$^{02}$ Eri	&		&	K0 V	&	Multiple	&	1	&	Dia18	\\
LP 714--47	&	J04167--120	&	M0.0 V	&	Single	&	1	&	Dre20	\\
PM J04343+4302	&	J04343+430	&	M2.5 V	&	Single	&	1	&	Blu21	\\
HD 29391	&		&	F0 V	&	Multiple	&	1	&	Mac15	\\
HD 285968	&	J04429+189	&	M2.0 V	&	Single	&	1	&	For09	\\
Wolf 1539	&	J04520+064	&	M3.5 V	&	Single	&	1	&	How10	\\
GJ 180	&	J04538--177	&	M2.0 V	&	Single	&	3	&	Tuo14	\\
GJ 3323	&	J05019--069	&	M4.0 V	&	Single	&	2	&	Ast17a	\\
GJ 229	&	J06105--218	&	M0.5 V	&	Multiple	&	2	&	Tuo14, Fen20	\\
HD 260655	&	J06371+175	&	M0.0 V	&	Single	&	2	&	Luq22	\\
HD 265866	&	J06548+332	&	M3.0 V	&	Single	&	1	&	Sto20b	\\
Luyten's Star	&	J07274+052	&	M3.5 V	&	Single	&	2	&	Ast17a, Poz20	\\
GJ 3470	&	J07590+153	&	M1.5 V	&	Single	&	1	&	Bon12	\\
GJ 3473	&	J08023+033	&	M4.0 V	&	Multiple	&	2	&	Kem20	\\
GJ 317	&	J08409--234	&	M3.5 V	&	Single	&	2	&	Joh07	\\
GJ 3512	&	J08413+594	&	M5.5 V	&	Single	&	2	&	Mor19	\\
$\rho^{01}$ Cnc	&		&	K0 IV/V	&	Multiple	&	5	&	But97, Mar02, Mc04, Fis08	\\
Ross 623	&	J08551+015	&	M0.0 V	&	Single	&	1	&	Rob13	\\
G 41--13	&	J08588+210	&	M2.0 V	&	Single	&	1	&	Stef20	\\
HD 79211	&	J09144+526	&	M0.0 V	&	Multiple	&	1	&	Gon20	\\
LP 727--31	&	J09286--121	&	M2.5 V	&	Single	&	1	&	Ree22	\\
GJ 357	&	J09360--216	&	M2.5 V	&	Single	&	3	&	Luq19	\\
GJ 378	&	J10023+480	&	M1.0 V	&	Single	&	1	&	Hob19	\\
TYC 4384--1735--1	&	J10088+692	&	M0.5 V	&	Single	&	1	&	Blu20, Clo20a	\\
LP 729--54	&	J10185--117	&	M4.0 V	&	Multiple	&	2	&	Now20, Clo20b	\\
Ross 446	&	J10289+008	&	M2.0 V	&	Single	&	1	&	Ama21	\\
Lalande 21185 	&	J11033+359	&	M1.5 V	&	Single	&	2	&	Dia19, Ros21	\\
HD 97101	&	J11110+304E	&	K7 V	&	Multiple	&	2	&	Ded21	\\
K2--18	&	J11302+076	&	M3.0 V	&	Single	&	1	&	FM15, Clo17, Sar18	\\
Ross 1003	&	J11417+427	&	M4.0 V	&	Single	&	2	&	Hag10, Tri18	\\
Ross 905	&	J11421+267	&	M2.5 V	&	Single	&	1	&	Butl04	\\
LP 375--23	&	J11423+230	&	M0.5 V	&	Multiple	&	1	&	Sta19	\\
FI Vir	&	J11477+008	&	M4.0 V	&	Single	&	1	&	Bon18a	\\
GJ 1151	&	J11509+483	&	M4.5 V	&	Single	&	1	&	Bla23	\\
HD 238090	&	J12123+544S	&	M0.0 V	&	Multiple	&	1	&	Sto20b	\\
Ross 690	&	J12230+640	&	M3.0 V	&	Single	&	1	&	End22	\\
Wolf 433	&	J12388+116	&	M3.0 V	&	Single	&	1	&	Fen20	\\
Wolf 437	&	J12479+097	&	M3.5 V	&	Single	&	1	&	Tri21	\\
PM J13119+6550	&	J13119+658	&	M3.0 V	&	Single	&	2	&	Dem20	\\
HD 115404	&		&	K2 V	&	Multiple	&	2	&	Fen22	\\
Ross 1020	&	J13229+244	&	M4.0 V	&	Single	&	1	&	Luq18	\\
TOI--1238	&	J13255+688	&	M0.0 V	&	Single	&	2	&	Gon22	\\
Ross 490	&	J13299+102	&	M0.5 V	&	Single	&	1	&	Dam22	\\
HD 122303	&	J14010--026	&	M1.0 V	&	Single	&	1	&	Sua17a	\\
HN Lib	&	J14342--125	&	M4.0 V	&	Single	&	1	&	Gon23a	\\
HO Lib	&	J15194--077	&	M3.0 V	&	Single	&	3	&	Bon05, May09, Udr07	\\
Ross 508	&	J15238+174	&	M4.5 V	&	Single	&	1	&	Har22	\\
GJ 3929	&	J15583+354	&	M3.5 V	&	Single	&	2	&	Kem22, Bea22	\\
GJ 3942	&	J16090+529	&	M0.0 V	&	Single	&	1	&	Per17	\\
K2--33	&	J16102--193	&	M3.0 V	&	Single	&	1	&	Dav16	\\
LP 804--27	&	J16126--188	&	M3.0 V	&	Single	&	1	&	App10	\\
HD 147379	&	J16167+672S	&	M0.0 V	&	Multiple	&	1	&	Rei18a	\\
GJ 625	&	J16254+543	&	M1.5 V	&	Single	&	1	&	Sua17b	\\
V2306 Oph	&	J16303--126	&	M3.5 V	&	Single	&	2	&	Wri16	\\
V1090 Her	&		&	K3 V	&	Multiple	&	3	&	Fen22	\\
Ross 860	&	J16581+257	&	M1.0 V	&	Single	&	1	&	Joh10	\\
GJ 1214	&	J17153+049	&	M4.5 V	&	Single	&	1	&	Cha09	\\
GJ 3998	&	J17160+110	&	M1.0 V	&	Single	&	2	&	Aff16	\\
GJ 685	&	J17355+616	&	M0.5 V	&	Multiple	&	1	&	Pin19	\\
GJ 687	&	J17364+683	&	M3.0 V	&	Single	&	2	&	Burt14	\\
GJ 686	&	J17378+185	&	M1.0 V	&	Single	&	1	&	Aff19	\\
GJ 720 A	&	J18353+457	&	M0.5 V	&	Multiple	&	1	&	Gon21	\\
LSPM J1835+3259	&	J18356+329	&	M8.5 V	&	Single	&	1	&	Ber17	\\
LP 141--14	&		&	DC	&	Multiple	&	1	&	Van20	\\
HD 176029	&	J18580+059	&	M0.5 V	&	Single	&	1	&	Tol21	\\
V1428 Aql	&	J19169+051N	&	M2.5 V	&	Multiple	&	1	&	Kam18	\\
2MASS J19204172+7311434	&	J19206+731S	&	M4.0 V	&	Multiple	&	1	&	Cad22	\\
HD 190360	&		&	G7 IV/V	&	Multiple	&	2	&	Nae03, Vog05	\\
Ross 754	&	J20138+133	&	M1.0 V	&	Single	&	1	&	Mal21	\\
Wolf 1069	&	J20260+585	&	M5.0 V	&	Single	&	1	&	Kos23	\\
AU Mic	&	J20451--313	&	M0.5 V	&	Multiple	&	2	&	Pla20, Mart21	\\
GJ 806	&	J20450+444	&	M1.5 V	&	Single	&	2	&	Pal23	\\
LSPM J2116+0234	&	J21164+025	&	M3.0 V	&	Single	&	1	&	Lal19	\\
TYC 2187--512--1	&	J21221+229	&	M1.0 V	&	Single	&	1	&	Qui22	\\
G 264--12	&	J21466+668	&	M4.0 V	&	Single	&	2	&	Ama21	\\
TYC 4266--736--1	&	J21474+627	&	M0.0 V	&	Multiple	&	1	&	Esp22	\\
Wolf 1329	&	J22096--046	&	M3.5 V	&	Single	&	2	&	Butl06, Mone14	\\
UCAC4 744--073158	&	J22102+587	&	M2.0 V	&	Single	&	1	&	Fuk22	\\
GJ 1265	&	J22137--176	&	M4.5 V	&	Single	&	1	&	Luq18	\\
GJ 4276	&	J22252+594	&	M4.0 V	&	Single	&	1	&	Nag19	\\
IL Aqr	&	J22532--142	&	M4.0 V	&	Single	&	4	&	Marc98, Mar01, Riv05, Riv10	\\
2MUCD 12171	&	J23064--050	&	M7.5 V	&	Single	&	7	&	Gil16, Gil17	\\
EQ Peg A	&	J23318+199E	&	M3.5 V	&	Multiple	&	1	&	Cur22	\\
\end{longtable}
\tablefoot{
\tablefoottext{a}{In the majority of cases these planets are classified as `Confirmed' (to the date of publication of this work) by the NASA Exoplanet Archive. A few controversial detections have been excluded (e.g. {Barnard's star} or CN Leo). Numbers in parenthesis denote that at least one planet has been challenged \citep{Rib23}.}
\tablefoottext{b}{References for the discovery -- 
Aff16: \cite{Aff16};
Aff19: \cite{Aff19};
Ama21: \cite{Ama21};
App10: \cite{App10};
Ast17a: \cite{Ast17a};
Ast17b: \cite{Ast17b};
Bau20: \cite{Bau20};
Bea22: \cite{Bea22};
Ber17: \cite{Ber17};
Bla23: \cite{Bla23};
Blu20: \cite{Blu20};
Blu21: \cite{Blu21};
Bon05: \cite{Bon05};
Bon12: \cite{Bon12};
Bon18a: \cite{Bon18a};
Burt14: \cite{Burt14};
But97: \cite{But97};
Butl04: \cite{Butl04};
Butl06: \cite{Butl06};
Cad22: \cite{Cad22};
Cha09: \cite{Cha09};
Cha22: \cite{Cha22};
Clo17: \cite{Clo17};
Clo20a: \cite{Clo20a};
Clo20b: \cite{Clo20b};
Cur22: \cite{Cur22};
Dam22: \cite{Dam22};
Dav16: \cite{Dav16};
Ded21: \cite{Ded21};
Dem20: \cite{Dem20};
Dho24: \cite{Dho24};
Dia18: \cite{Dia18};
Dia19: \cite{Dia19};
Dit17: \cite{Dit17};
Dre20: \cite{Dre20};
Dre24: \cite{Dre24};
End22: \cite{End22};
Esp22: \cite{Esp22};
FM15: \cite{FM15};
Fen20: \cite{Fen20};
Fen22: \cite{Fen22};
Fis08: \cite{Fis08};
For09: \cite{For09};
Fuk22: \cite{Fuk22};
Gil16: \cite{Gil16};
Gil17: \cite{Gil17};
Gon20: \cite{Gon20};
Gon21: \cite{Gon21};
Gon22: \cite{Gon22};
Gon23a: \cite{Gon23a};
Gon23b: \cite{Gon23b};
Hag10: \cite{Hag10};
Har22: \cite{Har22};
Hob19: \cite{Hob19};
How10: \cite{How10};
How14: \cite{How14};
Joh07: \cite{Joh07};
Joh10: \cite{Joh10};
Kam18: \cite{Kam18};
Kem20: \cite{Kem20};
Kem22: \cite{Kem22};
Kos21: \cite{Kos21};
Kos23: \cite{Kos23};
Kuz24: \cite{Kuz24};
Lal19: \cite{Lal19};
Luq18: \cite{Luq18};
Luq19: \cite{Luq19};
Luq22: \cite{Luq22};
Mac15: \cite{Mac15};
Mal21: \cite{Mal21};
Mar01: \cite{Mar01};
Mar02: \cite{Mar02};
Marc98: \cite{Marc98};
Mart21: \cite{Mart21};
May09: \cite{May09};
Mc04: \cite{Mc04};
Men19: \cite{Men19};
Mon14: \cite{Mon14};
Mor19: \cite{Mor19};
Nae03: \cite{Nae03};
Nag19: \cite{Nag19};
Now20: \cite{Now20};
Pal23: \cite{Pal23};
Per17: \cite{Per17};
Per19: \cite{Per19};
Pin18: \cite{Pin18};
Pin19: \cite{Pin19};
Pla20: \cite{Pla20};
Poz20: \cite{Poz20};
Qui22: \cite{Qui22};
Ree22: \cite{Ree22};
Rei18a: \cite{Rei18a};
Riv05: \cite{Riv05};
Riv10: \cite{Riv10};
Rob13: \cite{Rob13};
Ros21: \cite{Ros21};
Sar18: \cite{Sar18};
Sch21: \cite{Sch21};
Sot21: \cite{Sot21};
Sta19: \cite{Sta19};
Stef20: \cite{Stef20};
Sto20a: \cite{Sto20a};
Sto20b: \cite{Sto20b};
Sua17a: \cite{Sua17a};
Sua17b: \cite{Sua17b};
Sua23: \cite{Sua23};
Tol21: \cite{Tol21};
Tri18: \cite{Tri18};
Tri21: \cite{Tri21};
Tuo14: \cite{Tuo14};
Udr07: \cite{Udr07};
Van20: \cite{Van20};
Vog05: \cite{Vog05};
Win19b: \cite{Win19b};
Win22: \cite{Win22};
Wri16: \cite{Wri16};
Zec19: \cite{Zec19}.}
}



==> tables/table_new.tex <==
% Table: New candidates
\begin{landscape} 
\begin{longtable}{lllccccccc}
\caption{\label{tab:new} New stellar multiple systems not reported in the literature.}
\\
        \noalign{\smallskip}
        \noalign{\smallskip}
        \noalign{\smallskip}
\hline\hline
        \noalign{\smallskip}
Name	&	Karmn	&	Spectral	&	Component$^b$	&	$\alpha$	&	$\delta$	&	$\varpi$$^c$			&	$\mu_{\rm total}$			&	$\theta$	&	$\rho$	\\
	&		&	type$^a$	&		&		&		&	{[}mas{]}			&	{[}mas\,a$^{-1}${]}			&	{[}deg{]}	&	{[}arcsec{]}	\\
        \noalign{\smallskip}
\hline
        \noalign{\smallskip}
\endfirsthead
%
\caption{New stellar multiple systems not reported in the literature (continued).}\\
\hline\hline
        \noalign{\smallskip}
Name	&	Karmn	&	Spectral	&	Component$^b$	&	$\alpha$	&	$\delta$	&	$\varpi$$^c$			&	$\mu_{\rm total}$			&	$\theta$	&	$\rho$	\\
	&		&	type$^a$	&		&		&		&	{[}mas{]}			&	{[}mas\,a$^{-1}${]}			&	{[}deg{]}	&	{[}arcsec{]}	\\
\hline
        \noalign{\smallskip}
\endhead
%
\hline
\endfoot
        \noalign{\smallskip}
GJ 3261	&	J04056+057	&	M3.5 V	&	A	&	04:05:38.94	&	+05:44:40.4	&	16.094	$ \pm $	0.103	&	47.98	$ \pm $	0.15	&		&		\\
Gaia DR3 3296932486866670720	&		&	M4.0: V	&	B	&	04:05:38.89	&	+05:44:40.1	&				&				&	251.9	&	0.817	\\
V1221 Tau	&		&	M3.0: V	&	(C)	&	04:05:53.46	&	+05:31:24.6	&	15.876	$ \pm $	0.026	&	49.85	$ \pm $	0.03	&	164.8	&	824.8	\\
\noalign{\smallskip}        \noalign{\smallskip}																							
RX J0507.2+3731 A	&	J05072+375	&	M5.0 V	&	A	&	05:07:14.33	&	+37:30:42.1	&	43.800	$ \pm $	4.000	&	102.11	$ \pm $	4.90	&		&		\\
RX J0507.2+3731 B	&		&	M5.0: V 	&	(B)	&	05:07:14.37	&	+37:30:42.1	&	44.022	$ \pm $	0.461	&	96.09	$ \pm $	0.82	&	93.2	&	0.476	\\
\noalign{\smallskip}        \noalign{\smallskip}																							
LP 780--23	&	J06401--164	&	M2.5 V	&	A	&	06:40:08.72	&	--16:27:21.5	&		\ldots		&	319.03	$ \pm $	11.31	&		&		\\
LP 780--23 B	&		&	M2.5: V 	&	(B)	&	06:40:08.72	&	--16:27:21.7	&		\ldots		&		\ldots		&	187.9	&	0.199	\\
\noalign{\smallskip}        \noalign{\smallskip}																							
GJ 375.2	&	J10004+272	&	M0.5 V	&	A	&	10:00:26.69	&	+27:16:03.5	&	27.767	$ \pm $	0.016	&	118.42	$ \pm $	0.02	&		&		\\
2MASS J10003572+2717054	&		&	M6.5 V	&	B	&	10:00:35.70	&	+27:17:07.5	&	27.723	$ \pm $	0.103	&	118.34	$ \pm $	0.13	&	61.9	&	136.0	\\
Gaia DR3 740041664172917376	&		&	M7.5: V 	&	(C)	&	10:00:26.56	&	+27:16:05.7	&	26.561	$ \pm $	0.349	&	117.20	$ \pm $	0.34	&	320.9	&	2.882	\\
\noalign{\smallskip}        \noalign{\smallskip}																							
HD 230017 A$\dagger$	&		&	M0.0 V	&	A	&	18:54:53.67	&	+10:58:42.4	&	53.423	$ \pm $	0.108	&	133.27	$ \pm $	0.16	&		&		\\
HD 230017 B	&	J18548+109	&	M3.5 V	&	B	&	18:54:53.86	&	+10:58:45.1	&	53.644	$ \pm $	0.043	&	89.29	$ \pm $	0.06	&	45.1	&	3.792	\\
PM J18542+1058	&		&	M4.0 V	&	(C)	&	18:54:17.14	&	+10:58:11.0	&	53.838	$ \pm $	0.024	&	114.61	$ \pm $	0.03	&	266.7	&	538.9	\\
\noalign{\smallskip}        \noalign{\smallskip}																							
G 28--46 &	J23113+085	&	M3.0 V	&	A	&	23:11:23.45	&	+08:30:56.4	&	49.800	$ \pm $	3.300	&	458.92	$ \pm $	11.31	&		&		\\
G 28--46 B$\dagger$	&		&	M3.0: V 	&	(B)	&	23:11:23.47	&	+08:30:56.4	&		\ldots		&		\ldots		&	77.7	&	0.248	\\
\noalign{\smallskip}        \noalign{\smallskip}	
\end{longtable}
\tablefoot{
\tablefoottext{a}	{A colon (:) indicates an estimated spectral type from photometry.}
\tablefoottext{b}	{The new component found in each system is written in parentheses.}
\tablefoottext{$\dagger$} {
\object{HD~230017}\,ABC: Members of the Carina association \citep{Gag18b};
\object{G~28--46}\,AB: System identified as a close binary during the CARMENES exoplanet search \citep{Rib23}. A minimum period of 2225\,d was tabulated by \cite{Sab21} from spectroscopic observations.}
}
\end{landscape}



==> tables/table_outliers.tex <==
% Table: Outliers
\footnotesize{
\begin{longtable}{lcccccccc}
\caption{\label{tab:outliers} Components of multiple system that do not comply with one or more of the criteria for physical association.}
\\
        \noalign{\smallskip}
        \noalign{\smallskip}
        \noalign{\smallskip}
\hline\hline
        \noalign{\smallskip}
Name	& 	Comp.$^a$	& 	$\alpha$	&	$\delta$	&	$\mu$ ratio	& 	$\Delta PA$	& 	$\Delta d$	& 	$\rho^b$	& 	Cause$^c$	\\
	& 		& 	(J2016.0)	&	(J2016.0)	&		& 		& 		& 	{[}arcsec{]}	& 		\\
        \noalign{\smallskip}
\hline
        \noalign{\smallskip}
\endfirsthead
%
\caption{Components of multiple system that do not comply with one or more of the criteria for physical association (cont.).}\\
\hline\hline
        \noalign{\smallskip}
Name	& 	Comp.$^a$	& 	$\alpha$	&	$\delta$	&	$\mu$ ratio	& 	$\Delta PA$	& 	$\Delta d$	& 	$\rho^b$	& 	Cause$^c$	\\
	& 		& 	(J2016.0)	&	(J2016.0)	&		& 		& 		& 	{[}arcsec{]}	& 		\\
\hline
        \noalign{\smallskip}
\endhead
%
\hline
\endfoot
        \noalign{\smallskip}
PM J00026+3821 B	&	B	&	00:02:40.05	&	+38:21:45.3	&	0.214	&	12.254	&	0.031	&	1.415	&	1	\\
G 217--32 B	&	B	&	00:07:43.40	&	+60:22:53.8	&	0.196	&	9.161	&	0.0032	&	0.848	&	1	\\
LP 296--56	&	B	&	01:56:41.74	&	+30:28:34.6	&	0.012	&	0.027	&	0.163	&	299.1	&	3	\\
PM J02024+1034 A	&	B	&	02:02:28.18	&	+10:34:52.7	&	0.545	&	32.513	&	0.012	&	0.911	&	1	\\
LP 198--637 B	&	B	&	03:20:45.35	&	+39:42:59.6	&	0.152	&	8.738	&	0.0051	&	0.795	&	1	\\
PM J03247+4447 B	&	B	&	03:24:42.23	&	+44:47:39.7	&	0.191	&	4.590	&	0.0048	&	1.912	&	1	\\
Gaia DR3 3296932486866670720	&	B	&	04:05:38.89	&	+05:44:40.1	&	0.331	&	1.614	&	\ldots	&	0.817	&	1, 2	\\
GJ 2033 B	&	B	&	04:16:41.80	&	--12:33:19.8	&	0.334	&	11.137	&	0.0069	&	2.990	&	1	\\
HG 7--232 B	&	B	&	04:28:29.01	&	+17:41:45.3	&	0.227	&	11.403	&	0.047	&	1.663	&	1	\\
V697 Tau B	&	B	&	04:33:23.87	&	+23:59:26.5	&	0.200	&	11.095	&	0.150	&	0.767	&	1	\\
GJ 3305	&	BC	&	04:37:37.51	&	--02:29:29.7	&	0.274	&	14.659	&	0.077	&	0.098	&	1	\\
PM J04393+3331	&	BC	&	04:39:23.22	&	+33:31:48.7	&	0.147	&	7.913	&	0.333	&	0.126	&	1	\\
GJ 9163 B	&	B	&	04:40:29.15	&	--09:11:46.8	&	0.441	&	1.954	&	0.0064	&	1.715	&	1	\\
GJ 3322 B	&	B	&	05:01:58.89	&	+09:58:55.9	&	0.152	&	8.744	&	0.0015	&	1.398	&	1	\\
HD 32450 B	&	B	&	05:02:28.26	&	--21:15:27.5	&	0.247	&	6.461	&	0.0063	&	0.888	&	1	\\
LP 359--186	&	BC	&	05:03:05.77	&	+21:22:33.8	&	0.046	&	0.799	&	0.104	&	0.302	&	1, 2	\\
GJ 3332	&	B	&	05:06:49.48	&	--21:35:04.3	&	0.881	&	58.265	&	0.0018	&	8.489	&	1	\\
BD--21 1074 C	&	C	&	05:06:49.55	&	--21:35:04.7	&	0.309	&	8.384	&	0.0029	&	1.105	&	1	\\
GJ 3343	&	B	&	05:20:41.05	&	+58:47:12.0	&	0.021	&	1.037	&	0.104	&	14.11	&	3	\\
PM J05243--1601 B	&	B	&	05:24:19.17	&	--16:01:15.6	&	0.964	&	52.141	&	0.0066	&	0.444	&	1	\\
G 102--4 A	&	C	&	05:28:56.61	&	+12:31:50.4	&	0.023	&	1.307	&	0.169	&	99.39	&	2	\\
PM J05319--0303W	&	C	&	05:31:57.88	&	--03:03:37.6	&	0.254	&	4.659	&	0.034	&	150.0	&	1	\\
2MASS J05315816--0303397	&	D	&	05:31:58.17	&	--03:03:40.7	&	0.257	&	5.562	&	0.048	&	0.1	&	1	\\
ESO-HA  737	&	E	&	05:32:05.97	&	--03:01:16.8	&	0.209	&	5.090	&	0.046	&	254.2	&	1	\\
PM J06066+4633 B	&	B	&	06:06:37.77	&	+46:33:45.2	&	0.198	&	2.085	&	0.00038	&	1.790	&	1	\\
LP 362--121	&	B	&	06:10:22.52	&	+22:34:18.1	&	0.057	&	1.898	&	0.258	&	65.16	&	2	\\
Ross 603 B	&	B	&	06:27:43.74	&	+09:23:50.5	&	0.167	&	8.901	&	0.0052	&	1.170	&	1	\\
Gaia DR3 2926756741750933120	&	B	&	06:39:37.22	&	--21:01:31.9	&	0.590	&	11.207	&	0.025	&	0.556	&	1	\\
2MASS J07293670+3554531	&	C	&	07:29:36.67	&	+35:54:51.3	&	0.171	&	6.262	&	0.0063	&	95.88	&	3	\\
Castor C	&	Cab	&	07:34:37.19	&	+31:52:08.6	&	0.220	&	11.459	&	0.034	&	\ldots$\dagger$	&	1	\\
FP Cnc B	&	Cab	&	08:08:55.38	&	+32:49:01.4	&	0.189	&	10.740	&	0.022	&	\ldots$\dagger$	&	1	\\
GJ 1116 B	&	B	&	08:58:14.09	&	+19:45:45.3	&	0.236	&	5.329	&	0.011	&	2.175	&	1	\\
GJ 397.1 B	&	BC	&	10:31:30.64	&	+57:05:20.4	&	0.166	&	3.931	&	\ldots	&	0.284	&	1, 2	\\
PM J10367+1521 B	&	BC	&	10:36:44.92	&	+15:21:37.9	&	0.174	&	5.147	&	\ldots	&	0.858	&	1, 2	\\
GJ 3616 B	&	B	&	10:44:52.43	&	+32:24:40.1	&	0.067	&	2.466	&	0.129	&	1.296	&	1	\\
GJ 3617	&	C	&	10:44:54.79	&	+32:24:23.4	&	0.079	&	4.417	&	0.125	&	35.23	&	1, 2	\\
GJ 3628	&	B	&	10:50:37.91	&	+51:45:01.6	&	0.219	&	12.290	&	0.013	&	178.3	&	3	\\
HD 98712 B	&	B	&	11:21:26.84	&	--20:27:11.5	&	0.266	&	5.851	&	0.046	&	3.811	&	1	\\
GJ 426.1 B	&	B	&	11:23:55.75	&	+10:31:44.7	&	0.213	&	11.741	&	0.020	&	2.050	&	1	\\
Gaia DR3 3699797155055781760	&	B	&	12:20:25.60	&	+00:35:01.3	&	0.641	&	30.528	&	0.0055	&	0.882	&	1	\\
GJ 490 B	&	CD	&	12:57:38.94	&	+35:13:16.9	&	0.106	&	5.090	&	0.117	&	0.171	&	1	\\
PM J13260+2735 B	&	C	&	13:26:02.63	&	+27:35:02.5	&	0.201	&	8.729	&	0.0015	&	404.1	&	1	\\
GJ 520 B	&	B	&	13:37:50.77	&	+48:08:16.3	&	0.166	&	5.256	&	0.000046	&	1.621	&	1	\\
Gaia DR3 1658968054798747008	&	B	&	13:41:46.39	&	+58:15:18.6	&	0.360	&	13.784	&	0.0078	&	0.762	&	1	\\
GJ 536.1 B	&	B	&	14:01:58.89	&	+15:29:39.1	&	0.167	&	7.680	&	0.0020	&	1.621	&	1	\\
PM J14019+4316 B	&	B	&	14:01:58.69	&	+43:16:43.1	&	0.151	&	8.700	&	0.00081	&	1.960	&	1	\\
HD 124498 B	&	C	&	14:14:21.34	&	--15:21:24.4	&	0.175	&	9.130	&	0.077	&	1.553	&	1	\\
G 224--13 B	&	B	&	14:33:06.80	&	+61:00:43.6	&	0.190	&	10.854	&	0.0018	&	0.971	&	1	\\
GJ 9492 B	&	B	&	14:42:21.17	&	+66:03:20.1	&	0.221	&	11.795	&	0.0013	&	2.290	&	1	\\
GJ 569 B	&	BC	&	14:54:29.77	&	+16:06:05.6	&	0.215	&	7.832	&	0.067	&	\ldots$\dagger$	&	1	\\
Gaia DR3 1275127175448008448	&	B	&	15:18:49.78	&	+29:15:06.7	&	0.302	&	8.736	&	0.037	&	0.588	&	1	\\
Gaia DR3 1375767330164975616	&	B	&	15:33:54.89	&	+37:54:48.3	&	0.234	&	13.506	&	0.0022	&	0.834	&	1	\\
LP 331--57 B	&	B	&	17:03:53.14	&	+32:11:46.4	&	0.175	&	3.536	&	0.0055	&	1.393	&	1	\\
BD+19 3268 B	&	B	&	17:15:49.84	&	+19:00:00.3	&	0.699	&	3.435	&	0.0044	&	1.471	&	1	\\
RX J1734.0+4447 B	&	B	&	17:34:05.47	&	+44:47:08.4	&	0.403	&	17.500	&	0.058	&	0.633	&	1	\\
GJ 4021	&	C	&	17:38:40.87	&	+61:14:00.0	&	0.232	&	11.069	&	0.016	&	19.05	&	1	\\
GJ 695 C	&	D	&	17:46:24.65	&	+27:42:49.8	&	0.160	&	0.847	&	0.0039	&	0.575	&	1	\\
HD 230017 B	&	B	&	18:54:53.86	&	+10:58:45.1	&	0.512	&	6.480	&	0.0041	&	3.792	&	1	\\
PM J18542+1058	&	C	&	18:54:17.14	&	+10:58:11.0	&	0.170	&	2.601	&	0.0078	&	538.9	&	1	\\
StKM 1--1676 B	&	C	&	19:03:17.96	&	+63:59:37.4	&	0.824	&	54.189	&	\ldots	&	3.578	&	1	\\
GJ 4115	&	C	&	19:35:06.33	&	+08:27:43.4	&	0.462	&	17.584	&	0.062	&	5.635	&	1	\\
GJ 1245 B	&	C	&	19:53:55.66	&	+44:24:46.5	&	0.174	&	9.449	&	0.0068	&	5.945	&	1	\\
LP 395--8 B	&	B	&	20:19:49.35	&	+22:56:40.0	&	0.184	&	10.601	&	0.000044	&	1.918	&	1	\\
GJ 4153 B	&	B	&	20:37:23.97	&	+21:56:21.4	&	0.072	&	0.221	&	0.217	&	51.77	&	2	\\
AT Mic B	&	C	&	20:41:51.54	&	--32:26:15.1	&	0.298	&	13.947	&	0.012	&	2.102	&	1	\\
PM J21055+0609S	&	B	&	21:05:32.17	&	+06:09:11.2	&	0.175	&	5.680	&	0.000069	&	5.094	&	1	\\
DENIS J210844.8--042517	&	C	&	21:08:44.75	&	--04:25:18.3	&	0.652	&	12.094	&	0.012	&	20.89	&	1	\\
GJ 4188	&	C	&	21:17:39.55	&	--08:54:49.6	&	0.166	&	7.927	&	0.098	&	63.99	&	1	\\
GJ 4201 B	&	B	&	21:32:22.23	&	+24:33:41.1	&	0.181	&	9.559	&	0.0029	&	1.548	&	1	\\
GJ 834 B	&	B	&	21:36:38.20	&	+39:27:17.8	&	0.181	&	9.172	&	0.0041	&	1.003	&	1	\\
UCAC4 747--070768	&	B	&	21:51:39.93	&	+59:17:34.5	&	0.384	&	20.069	&	0.041	&	14.64	&	1	\\
LP 759--25	&	B	&	22:05:35.44	&	--11:04:31.8	&	0.053	&	3.002	&	0.323	&	3030.6	&	3	\\
Wolf 1225 B	&	B	&	22:23:29.34	&	+32:27:29.5	&	0.271	&	12.352	&	0.0040	&	1.252	&	1	\\
DO Cep	&	B	&	22:27:57.93	&	+57:41:38.8	&	0.438	&	19.178	&	0.0023	&	2.052	&	1	\\
GJ 4282 B	&	B	&	22:33:22.87	&	--09:36:53.7	&	0.172	&	5.466	&	0.0022	&	1.399	&	1	\\
2MASS J23301129--0237227	&	B	&	23:30:11.41	&	--02:37:23.9	&	0.069	&	3.658	&	0.232	&	1469.1	&	3	\\
EQ Peg B	&	B	&	23:31:53.20	&	+19:56:14.3	&	0.152	&	8.006	&	0.0015	&	5.376	&	1	\\
GJ 897	&	C	&	23:32:46.98	&	--16:45:12.3	&	0.938	&	66.572	&	\ldots$\dagger$	&	337.9	&	2	\\
\end{longtable}
\tablefoot{
\tablefoottext{a}	{Component in system.}
\tablefoottext{b}	{Angular separation of the closest component.}
\tablefoottext{c}	{Cause of the deviation: 
1:	Presence of a very close companion (either resolved or not). This is also applicable to the primary;
2:	Distances and proper motions from a source different than {\em Gaia} DR3, with larger uncertainties, or missing values;
3: New unresolved binary candidates as described in Sect.~\ref{ssection:candidates}. This is applicable to the primary.
}
\tablefoottext{$\dagger$}	{
\object{Castor~C}: Detached eclipsing double-lined spectroscopic binary (DESB2) with $a\lesssim$ 0.01\,au \citep{Tor02};  
\object{FP~Cnc~B}: SB2 \citep{Shk10} in a quadruple system;
\object{GJ~569~B}: Ultra-cool companion resolved ($\rho \lesssim$ 0.1\,arcsec) with the Keck Adaptive Optics Facility \citep{Mar00,Lan01}; 
\object{GJ~897}: Parallax from Hipparcos removed because of extremely large relative error.
}
}
}

==> tables/table_references.tex <==
\begin{longtable}{llllll}
\caption{\label{tab:references} Bibliographic references for the abbreviations used in the main table.}\\
\noalign{\smallskip}
\hline\hline
\noalign{\smallskip} 
Abbreviation	& 	Reference	& 	Abbreviation	& 	Reference	& 	Abbreviation	& 	Reference	\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
\endfirsthead
\caption{Bibliographic references for the abbreviations used in the main table (cont.).}\\
\hline\hline
\noalign{\smallskip}        
Abbreviation 	& 	Reference	& 	Abbreviation	& 	Reference	& 	Abbreviation	& 	Reference	\\
\hline
\noalign{\smallskip}
\endhead
%
\hline
\endfoot
\noalign{\smallskip}
Abt08	&	\cite{Abt08}	&	Can93	&	\cite{Can93}	&	Fen20	&	\cite{Fen20}	\\
Abt70	&	\cite{Abt70}	&	Car21	&	\cite{Car21}	&	Fen22	&	\cite{Fen22}	\\
Abt76	&	\cite{Abt76}	&	Cas07	&	\cite{Cas07}	&	Fin18	&	\cite{Fin18}	\\
Abt81	&	\cite{Abt81}	&	Cat06	&	\cite{Cat06}	&	Fis08	&	\cite{Fis08}	\\
Ada35	&	\cite{Ada35}	&	Cha09	&	\cite{Cha09}	&	Fle88	&	\cite{Fle88}	\\
Aff16	&	\cite{Aff16}	&	Cha22	&	\cite{Cha22}	&	FM15	&	\cite{FM15}	\\
Aff19	&	\cite{Aff19}	&	Che20	&	\cite{Che20}	&	For04	&	\cite{For04}	\\
Alo15a	&	\cite{Alo15a}	&	Che23	&	\cite{Che23}	&	For09	&	\cite{For09}	\\
Alo15b	&	\cite{Alo15b}	&	Chr38	&	\cite{Chr38}	&	Fou18	&	\cite{Fou18}	\\
Ama21	&	\cite{Ama21}	&	Chr78	&	\cite{Chr78}	&	Fre20	&	\cite{Fre20}	\\
Ans15	&	\cite{Ans15}	&	Cif20	&	\cite{Cif20}	&	Fri13	&	\cite{Fri13}	\\
App10	&	\cite{App10}	&	Clo03	&	\cite{Clo03}	&	Fuk22	&	\cite{Fuk22}	\\
Are19	&	\cite{Are19}	&	Clo17	&	\cite{Clo17}	&	Gag15a	&	\cite{Gag15a}	\\
Ast17a	&	\cite{Ast17a}	&	Clo20a	&	\cite{Clo20a}	&	Gag18a	&	\cite{Gag18a}	\\
Ast17b	&	\cite{Ast17b}	&	Clo20b	&	\cite{Clo20b}	&	Gag18b	&	\cite{Gag18b}	\\
Bar14	&	\cite{Bar14}	&	Cor17a	&	\cite{Cor17a}	&	Gai14b	&	\cite{Gai14b}	\\
Bar18	&	\cite{Bar18}	&	Cor24	&	\cite{Cor24}	&	Gaia22a	&	\cite{Gaia22a}	\\
Bar21	&	\cite{Bar21}	&	Cru02	&	\cite{Cru02}	&	Gal22	&	\cite{Gal22}	\\
Bar70	&	\cite{Bar70}	&	Cru03	&	\cite{Cru03}	&	Geb02	&	\cite{Geb02}	\\
Bau20	&	\cite{Bau20}	&	Cru09	&	\cite{Cru09}	&	Geb16	&	\cite{Geb16}	\\
Bea22	&	\cite{Bea22}	&	Cur06	&	\cite{Cur06}	&	Gen19	&	\cite{Gen19}	\\
Bed20	&	\cite{Bed20}	&	Cur22	&	\cite{Cur22}	&	Gia11	&	\cite{Gia11}	\\
Bel17	&	\cite{Bel17}	&	Cve12	&	\cite{Cve12}	&	Gil16	&	\cite{Gil16}	\\
Bel97	&	\cite{Bel97}	&	Dae07	&	\cite{Dae07}	&	Gil17	&	\cite{Gil17}	\\
Ben00	&	\cite{Ben00}	&	Dam22	&	\cite{Dam22}	&	Gil18	&	\cite{Gil18}	\\
Ben08	&	\cite{Ben08}	&	Dav14	&	\cite{Dav14}	&	Giz00b	&	\cite{Giz00b}	\\
Ben21	&	\cite{Ben21}	&	Dav15	&	\cite{Dav15}	&	Giz02	&	\cite{Giz02}	\\
Ber06	&	\cite{Ber06}	&	Dav16	&	\cite{Dav16}	&	Giz97a	&	\cite{Giz97a}	\\
Ber10	&	\cite{Ber10}	&	Daw05	&	\cite{Daw05}	&	Giz97b	&	\cite{Giz97b}	\\
Ber17	&	\cite{Ber17}	&	Dea12	&	\cite{Dea12}	&	Gli91	&	\cite{Gli91}	\\
Bes15	&	\cite{Bes15}	&	Dea14	&	\cite{Dea14}	&	Gol10	&	\cite{Gol10}	\\
Bes20	&	\cite{Bes20}	&	Ded21	&	\cite{Ded21}	&	Gom15	&	\cite{Gom15}	\\
Bes91	&	\cite{Bes91}	&	Dek18	&	\cite{Dek18}	&	Gon06	&	\cite{Gon06}	\\
Bid85	&	\cite{Bid85}	&	Del10	&	\cite{Del10}	&	Gon20	&	\cite{Gon20}	\\
Bil13	&	\cite{Bil13}	&	Del98	&	\cite{Del98}	&	Gon21	&	\cite{Gon21}	\\
Bin16	&	\cite{Bin16}	&	Del99a	&	\cite{Del99b}	&	Gon22	&	\cite{Gon22}	\\
Bir12	&	\cite{Bir12}	&	Del99b	&	\cite{Del99a}	&	Gon23a	&	\cite{Gon23a}	\\
Bir20	&	\cite{Bir20}	&	Del99c	&	\cite{Del99c}	&	Gon23b	&	\cite{Gon23b}	\\
Bla23	&	\cite{Bla23}	&	Dem20	&	\cite{Dem20}	&	Gon24	&	\cite{Gon24}	\\
Blu20	&	\cite{Blu20}	&	Des12	&	\cite{Des12}	&	GR96	&	\cite{GR96}	\\
Blu21	&	\cite{Blu21}	&	Dho24	&	\cite{Dho24}	&	Gra01	&	\cite{Gra01}	\\
Boc05	&	\cite{Boc05}	&	Dia18	&	\cite{Dia18}	&	Gra03	&	\cite{Gra03}	\\
Boc18	&	\cite{Boc18}	&	Dia19	&	\cite{Dia19}	&	Gra06	&	\cite{Gra06}	\\
Bon05	&	\cite{Bon05}	&	Die14	&	\cite{Die14}	&	Gre84	&	\cite{Gre84}	\\
Bon12	&	\cite{Bon12}	&	Dit14	&	\cite{Dit14}	&	Gre90	&	\cite{Gre90}	\\
Bon13a	&	\cite{Bon13a}	&	Dit17	&	\cite{Dit17}	&	Gri85	&	\cite{Gri85}	\\
Bon18a	&	\cite{Bon18a}	&	DR2	&	\cite{Gaia18bro}	&	Gui09	&	\cite{Gui09}	\\
Bop77	&	\cite{Bop77}	&	DR3	&	\cite{Gaia23}	&	Hag10	&	\cite{Hag10}	\\
Bow15a	&	\cite{Bow15a}	&	Dre19	&	\cite{Dre19}	&	Hal18	&	\cite{Hal18}	\\
Bud19	&	\cite{Bud19}	&	Dre20	&	\cite{Dre20}	&	Har11	&	\cite{Har11}	\\
Bud21	&	\cite{Bud21}	&	Dre24	&	\cite{Dre24}	&	Har12	&	\cite{Har12}	\\
Bur00	&	\cite{Bur00}	&	Dup12	&	\cite{Dup12}	&	Har22	&	\cite{Har22}	\\
Bur11	&	\cite{Bur11}	&	Dup17	&	\cite{Dup17}	&	Har70	&	\cite{Har70}	\\
Bur13	&	\cite{Bur13}	&	Dup19	&	\cite{Dup19}	&	Har81	&	\cite{Har81}	\\
Bur15a	&	\cite{Bur15a}	&	Dup94	&	\cite{Dup94}	&	Har96	&	\cite{Har96}	\\
Bur15b	&	\cite{Bur15b}	&	Duq88	&	\cite{Duq88}	&	Haw96	&	\cite{Haw96}	\\
Burt14	&	\cite{Burt14}	&	Duq91	&	\cite{Duq91}	&	Hen02	&	\cite{Hen02}	\\
But97	&	\cite{But97}	&	Edw76	&	\cite{Edw76}	&	Hen18	&	\cite{Hen18}	\\
Butl04	&	\cite{Butl04}	&	Ell14	&	\cite{Ell14}	&	Her03	&	\cite{Her03}	\\
Butl06	&	\cite{Butl06}	&	End22	&	\cite{End22}	&	Her14	&	\cite{Her14}	\\
Cab07	&	\cite{Cab07}	&	Esp22	&	\cite{Esp22}	&	Her65	&	\cite{Her65}	\\
Cab09	&	\cite{Cab09}	&	Eva67	&	\cite{Eva67}	&	Hir21	&	\cite{Hir21}	\\
Cab10a	&	\cite{Cab10a}	&	Fab02	&	\cite{Fab02}	&	Hob19	&	\cite{Hob19}	\\
Cab10b	&	\cite{Cab10b}	&	Fah10	&	\cite{Fah10}	&	Hog00	&	\cite{Hog00}	\\
Cad22	&	\cite{Cad22}	&	Fah12	&	\cite{Fah12}	&	Hoj19	&	\cite{Hoj19}	\\
										
Hou16	&	\cite{Hou16}	&	Luc17	&	\cite{Luc17}	&	Pha06a	&	\cite{Pha06a}	\\
Hou88	&	\cite{Hou88}	&	Luc18	&	\cite{Luc18}	&	Pha06b	&	\cite{Pha06b}	\\
Hou99	&	\cite{Hou99}	&	Luh12	&	\cite{Luh12}	&	Pin18	&	\cite{Pin18}	\\
How10	&	\cite{How10}	&	Luq18	&	\cite{Luq18}	&	Pin19	&	\cite{Pin19}	\\
How14	&	\cite{How14}	&	Luq19	&	\cite{Luq19}	&	Pla20	&	\cite{Pla20}	\\
Hub22	&	\cite{Hub22}	&	Luq22	&	\cite{Luq22}	&	Pou04	&	\cite{Pou04}	\\
Ire08	&	\cite{Ire08}	&	Mac13	&	\cite{Mac13}	&	Poz20	&	\cite{Poz20}	\\
Irw09	&	\cite{Irw09}	&	Mac15	&	\cite{Mac15}	&	Pre02	&	\cite{Pre02}	\\
Jah08	&	\cite{Jah08}	&	Mac18	&	\cite{Mac18}	&	Put97	&	\cite{Put97}	\\
Jam08	&	\cite{Jam08}	&	Mah21	&	\cite{Mah21}	&	Qui22	&	\cite{Qui22}	\\
Jan12	&	\cite{Jan12}	&	Mal06	&	\cite{Mal06}	&	Rag09	&	\cite{Rag09}	\\
Jan14a	&	\cite{Jan14a}	&	Mal12	&	\cite{Mal12}	&	Raj18a	&	\cite{Raj18a}	\\
Jan17	&	\cite{Jan17}	&	Mal13	&	\cite{Mal13}	&	Reb98	&	\cite{Reb98}	\\
Jef18	&	\cite{Jef18}	&	Mal14a	&	\cite{Mal14a}	&	Ree22	&	\cite{Ree22}	\\
Jen09	&	\cite{Jen09}	&	Mal14b	&	\cite{Mal14b}	&	Rei02a	&	\cite{Rei02a}	\\
Jim18	&	\cite{Jim18}	&	Mal20	&	\cite{Mal20}	&	Rei03	&	\cite{Rei03}	\\
Jod13	&	\cite{Jod13}	&	Mal21	&	\cite{Mal21}	&	Rei04	&	\cite{Rei04}	\\
Joh07	&	\cite{Joh07}	&	Mal24	&	\cite{Mal24}	&	Rei05	&	\cite{Rei05}	\\
Joh10	&	\cite{Joh10}	&	Man14	&	\cite{Man14}	&	Rei07	&	\cite{Rei07}	\\
Jon20	&	\cite{Jon20}	&	Man15	&	\cite{Man15}	&	Rei09	&	\cite{Rei09}	\\
Joy26	&	\cite{Joy26}	&	Mar01	&	\cite{Mar01}	&	Rei18a	&	\cite{Rei18a}	\\
Joy49	&	\cite{Joy49}	&	Mar02	&	\cite{Mar02}	&	Rei18b	&	\cite{Rei18b}	\\
Joy74	&	\cite{Joy74}	&	Mar07	&	\cite{Mar07}	&	Rei95	&	\cite{Rei95}	\\
Kam18	&	\cite{Kam18}	&	Mar87	&	\cite{Mar87}	&	Rei97b	&	\cite{Rei97b}	\\
Kar04	&	\cite{Kar04}	&	Marc98	&	\cite{Marc98}	&	Rein12	&	\cite{Rein12}	\\
Kat13	&	\cite{Kat13}	&	Marf21	&	\cite{Marf21}	&	Ria06	&	\cite{Ria06}	\\
Kee89	&	\cite{Kee89}	&	Mart21	&	\cite{Mart21}	&	Rib23	&	\cite{Rib23}	\\
Kem20	&	\cite{Kem20}	&	Mas08	&	\cite{Mas08}	&	Ric20	&	\cite{Ric20}	\\
Kem22	&	\cite{Kem22}	&	May09	&	\cite{May09}	&	Rie17	&	\cite{Rie17}	\\
Ker19	&	\cite{Ker19}	&	Maz01	&	\cite{Maz01}	&	Riv05	&	\cite{Riv05}	\\
Khr10	&	\cite{Khr10}	&	Mc04	&	\cite{Mc04}	&	Riv10	&	\cite{Riv10}	\\
Kir11	&	\cite{Kir11}	&	McC02	&	\cite{McC02}	&	Riv12	&	\cite{Riv12}	\\
Kir12	&	\cite{Kir12}	&	Men19	&	\cite{Men19}	&	Rob12	&	\cite{Rob12}	\\
Kir19	&	\cite{Kir19}	&	Mer09	&	\cite{Mer09}	&	Rob13	&	\cite{Rob13}	\\
Kir24	&	\cite{Kir24}	&	Mir20	&	\cite{Mir20}	&	Rod74	&	\cite{Rod74}	\\
Kir91	&	\cite{Kir91}	&	Mis15	&	\cite{Mis15}	&	Roj12	&	\cite{Roj12}	\\
Kir94	&	\cite{Kir94}	&	Moc02	&	\cite{Moc02}	&	Ros11	&	\cite{Ros11}	\\
Kiy20	&	\cite{Kiy20}	&	Mon01	&	\cite{Mon01}	&	Ros21	&	\cite{Ros21}	\\
Klu20	&	\cite{Klu20}	&	Mon03	&	\cite{Mon03}	&	Sab21	&	\cite{Sab21}	\\
Koe10	&	\cite{Koe10}	&	Mon14	&	\cite{Mon14}	&	Sal22	&	\cite{Sal22}	\\
Kop16	&	\cite{Kop16}	&	Mon18	&	\cite{Mon18}	&	Sam17	&	\cite{Sam17}	\\
Kos21	&	\cite{Kos21}	&	Mor09	&	\cite{Mor09}	&	Sar18	&	\cite{Sar18}	\\
Kos23	&	\cite{Kos23}	&	Mor10	&	\cite{Mor10}	&	Sch05	&	\cite{Sch05}	\\
Kou19	&	\cite{Kou19}	&	Mor19	&	\cite{Mor19}	&	Sch07	&	\cite{Sch07}	\\
Kra14a	&	\cite{Kra14a}	&	Mor65	&	\cite{Mor65}	&	Sch12	&	\cite{Sch12}	\\
Kra14b	&	\cite{Kra14b}	&	Mut10	&	\cite{Mut10}	&	Sch19	&	\cite{Sch19}	\\
Kra17	&	\cite{Kra17}	&	MWDD	&	Montreal WD Database	&	Sch21	&	\cite{Sch21}	\\
Kuz19	&	\cite{Kuz19}	&	Nae03	&	\cite{Nae03}	&	Scha19	&	\cite{Scha19}	\\
Kuz24	&	\cite{Kuz24}	&	Nag19	&	\cite{Nag19}	&	Schw19	&	\cite{Schw19}	\\
Lafr07	&	\cite{Lafr07}	&	Nap20	&	\cite{Nap20}	&	She85	&	\cite{She85}	\\
Lal19	&	\cite{Lal19}	&	Nes95	&	\cite{Nes95}	&	Shk09	&	\cite{Shk09}	\\
Law06	&	\cite{Law06}	&	New14	&	\cite{New14}	&	Shk10	&	\cite{Shk10}	\\
Law08	&	\cite{Law08}	&	New16	&	\cite{New16}	&	Shk12	&	\cite{Shk12}	\\
Lee84	&	\cite{Lee84}	&	Nid02	&	\cite{Nid02}	&	Shk17	&	\cite{Shk17}	\\
Lep02	&	\cite{Lep02}	&	Now20	&	\cite{Now20}	&	Sim11	&	\cite{Sim11}	\\
Lep03	&	\cite{Lep03}	&	Osw88	&	\cite{Osw88}	&	Sio09	&	\cite{Sio09}	\\
Lep05	&	\cite{Lep05}	&	Pal20	&	\cite{Pal20}	&	Sio90	&	\cite{Sio90}	\\
Lep09	&	\cite{Lep09}	&	Pal23	&	\cite{Pal23}	&	Ski18	&	\cite{Ski18}	\\
Lep13	&	\cite{Lep13}	&	Pas18	&	\cite{Pas18}	&	Smi14	&	\cite{Smi14}	\\
Lim13	&	\cite{Lim13}	&	Pau06	&	\cite{Pau06}	&	Sot21	&	\cite{Sot21}	\\
Lim15	&	\cite{Lim15}	&	Pec13	&	\cite{Pec13}	&	Sou18	&	\cite{Sou18}	\\
Lod05	&	\cite{Lod05}	&	Per17	&	\cite{Per17}	&	Soub08	&	\cite{Soub08}	\\
Lod19	&	\cite{Lod19}	&	Per19	&	\cite{Per19}	&	Spe16	&	\cite{Spe16}	\\
Lop06	&	\cite{Lop06}	&	Pes97	&	\cite{Pes97}	&	Spe19	&	\cite{Spe19}	\\
Lot98	&	\cite{Lot98}	&	Pet84	&	\cite{Pet84}	&	Spi21	&	\cite{Spi21}	\\
											
Sta19	&	\cite{Sta19}	&	Tok18	&	\cite{Tok18}	&	War15	&	\cite{War15}	\\
Sta97	&	\cite{Sta97}	&	Tok22	&	\cite{Tok22}	&	Wei16	&	\cite{Wei16}	\\
Ste86a	&	\cite{Ste86a}	&	Tok97	&	\cite{Tok97}	&	Wes11	&	\cite{Wes11}	\\
Ste86b	&	\cite{Ste86b}	&	Tol21	&	\cite{Tol21}	&	Wes93	&	\cite{Wes93}	\\
Stef20	&	\cite{Stef20}	&	Tor02	&	\cite{Tor02}	&	Whi01	&	\cite{Whi01}	\\
Stei20	&	\cite{Stei20}	&	Tor06	&	\cite{Tor06}	&	Whi07	&	\cite{Whi07}	\\
Sto20a	&	\cite{Sto20a}	&	Tor09	&	\cite{Tor09}	&	Wil53	&	\cite{Wil53}	\\
Sto20b	&	\cite{Sto20b}	&	Tor10	&	\cite{Tor10}	&	Win17	&	\cite{Win17}	\\
Ston20	&	\cite{Ston20}	&	Tor22	&	\cite{Tor22}	&	Win19b	&	\cite{Win19b}	\\
Str03	&	\cite{Str03}	&	TP86	&	\cite{TP86}	&	Win20	&	\cite{Win20}	\\
Str93	&	\cite{Str93}	&	Tre20	&	\cite{Tre20}	&	Win22	&	\cite{Win22}	\\
Str94	&	\cite{Str94}	&	Tri18	&	\cite{Tri18}	&	Wri16	&	\cite{Wri16}	\\
Sua17a	&	\cite{Sua17a}	&	Tri21	&	\cite{Tri21}	&	Xua24	&	\cite{Xua24}	\\
Sua17b	&	\cite{Sua17b}	&	Tuo14	&	\cite{Tuo14}	&	Yi14	&	\cite{Yi14}	\\
Sua23	&	\cite{Sua23}	&	Udr07	&	\cite{Udr07}	&	Zac10	&	\cite{Zac10}	\\
Tab17	&	\cite{Tab17}	&	van07	&	\cite{van07}	&	Zac12	&	\cite{Zac12}	\\
Tam06	&	\cite{Tam06}	&	van09	&	\cite{van09}	&	Zak22	&	\cite{Zak22}	\\
Tam08	&	\cite{Tam08}	&	Van20	&	\cite{Van20}	&	Zak79	&	\cite{Zak79}	\\
Tau20	&	\cite{Tau20}	&	van95	&	\cite{van95}	&	Zap04	&	\cite{Zap04}	\\
Ter15a	&	\cite{Ter15a}	&	Vog02	&	\cite{Vog02}	&	Zbo98	&	\cite{Zbo98}	\\
Ter15b	&	\cite{Ter15b}	&	Vog05	&	\cite{Vog05}	&	Zec19	&	\cite{Zec19}	\\
Tin19	&	\cite{Tin19}	&	Vri20	&	\cite{Vri20}	&	Zon20	&	\cite{Zon20}	\\
Tok08	&	\cite{Tok08}	&	Wan22	&	\cite{Wan22}	&		&		\\
\end{longtable}

==> tables/table_widest.tex <==
{\fontsize{7}{10}\selectfont 
\begin{landscape}
\begin{longtable}{lllllcccccll}
\caption{Multiple systems with components at separations larger than 10$^4$\,au.}
\label{tab:widest} 
\\
\hline\hline \noalign{\smallskip}
Name	& 	Karmn	& 	Spectral	& 	Comp.	& 	Discoverer$^a$	& 	$s$ {[}au{]}		& 	$\pi$			& 	$\mu_{\rm total}$			& 	$|U^\ast_g|$			& 	SKG	& 	SKG	\\
	& 		& 	type	& 		& 		& 			& 	{[}mas{]}			& 	{[}mas\,a$^{-1}${]}			& 	{[}$10^{33}$\,J{]}			& 		& 	Ref.$^b$	\\
\noalign{\smallskip}
\hline \noalign{\smallskip}
\endfirsthead
\caption{Multiple systems with components at separations larger than 10$^4$\,au. (cont.).}\\
\hline\hline 
\noalign{\smallskip}
Name	& 	Karmn	& 	Spectral	& 	Comp.	& 	Discoverer$^a$	& 	$s$ {[}au{]}		& 	$\pi$			& 	$\mu_{\rm total}$			& 	$|U^\ast_g|$			& 	SKG	& 	SKG	\\
	& 		& 	type	& 		& 		& 			& 	{[}mas{]}			& 	{[}mas\,a$^{-1}${]}			& 	{[}$10^{33}$\,J{]}			& 		& 	Ref.$^b$	\\
\hline \noalign{\smallskip}
\endhead
\hline
\endfoot
\noalign{\smallskip}
GJ 3022	&	J00169+200	&	M3.5 V	&	A	&		&			&	29.310	 $\pm$ 	0.097	&	239.537	 $\pm$ 	0.209	&				&		&		\\
G 131--47 B	&		&	M3.5 V	&	B	&	CRC 43	&	36.96		&	29.139	 $\pm$ 	0.071	&	233.362	 $\pm$ 	0.318	&	4764	 $\pm$ 	727	&		&		\\
LP 404--54	&		&	M5.0 V	&	C	&	Sma21	&	60679.5		&	28.873	 $\pm$ 	0.034	&	233.800	 $\pm$ 	0.048	&	1.742	 $\pm$ 	0.211	&		&		\\
\noalign{\smallskip}        \noalign{\smallskip}																												
V493 And A	&	J00341+253	&	M0.0 V	&	A	&		&			&	20.101	 $\pm$ 	0.039	&	127.914	 $\pm$ 	0.054	&				&	AB Dor	&	Jan17	\\
V493 And B	&		&	K7 V	&	B	&	SKF 220	&	77.91		&	19.720	 $\pm$ 	0.037	&	129.463	 $\pm$ 	0.056	&	10445	 $\pm$ 	567	&	AB Dor	&	$\star$	\\
UCAC4 578--001365	&		&	M4.0 V	&	C	&	Sma21	&	15617.5		&	19.672	 $\pm$ 	0.234	&	127.043	 $\pm$ 	0.353	&	20.44	 $\pm$ 	1.29	&	AB Dor	&	$\star$	\\
\noalign{\smallskip}        \noalign{\smallskip}																												
EX Cet	&		&	K0.5 V	&	A	&		&			&	41.564	 $\pm$ 	0.024	&	197.856	 $\pm$ 	0.032	&				&	Ple/beta Pic	&	$\star$	\\
LP 648--20$^c$	&	J01369--067	&	M3.5 V	&	B	&	CAB 3	&	14678.4		&	41.699	 $\pm$ 	0.045	&	200.547	 $\pm$ 	0.052	&	34.09	 $\pm$ 	5.33	&	Ple/beta Pic	&	Alo15b	\\
\noalign{\smallskip}        \noalign{\smallskip}																												
G 221--21	&	J03454+729	&	M1.5 V	&	A	&		&			&	39.088	 $\pm$ 	0.013	&	487.290	 $\pm$ 	0.016	&				&		&		\\
LP 31--200	&		&	M3.5 V	&	B	&	WIS  99	&	14667.0		&	39.146	 $\pm$ 	0.015	&	488.277	 $\pm$ 	0.018	&	14.70	 $\pm$ 	1.08	&		&		\\
\noalign{\smallskip}        \noalign{\smallskip}																												
LSPM J0401+5131	&		&	DC8	&	A	&		&			&	39.836	 $\pm$ 	0.077	&	883.245	 $\pm$ 	0.117	&				&		&		\\
Ross 25	&	J04011+513	&	M3.5 V	&	B	&	Sma21	&	12401.7		&	39.816	 $\pm$ 	0.021	&	883.463	 $\pm$ 	0.028	&	23.97	 $\pm$ 	4.90	&		&		\\
\noalign{\smallskip}        \noalign{\smallskip}																												
GJ 3261	&	J04056+057	&	M3.5 V	&	A	&		&			&	16.094	 $\pm$ 	0.103	&	47.984	 $\pm$ 	0.155	&				&	beta Pic	&	Gag18b	\\
G3 3296932486866670720	&		&	M4.0 V	&	B	&	MCT   3	&			&		\ldots		&		\ldots		&				&	beta Pic	&	$\star$	\\
V1221 Tau	&		&	M3.0 V	&	C	&	This work	&	51950.3		&	15.876	 $\pm$ 	0.026	&	49.854	 $\pm$ 	0.034	&	10.56	 $\pm$ 	0.62	&	beta Pic	&	Gag18b	\\
\noalign{\smallskip}        \noalign{\smallskip}																												
LP 414--117	&	J04123+162	&	M4.0 V	&	Aab	&	Ben08	&			&	28.240	 $\pm$ 	0.091	&	156.844	 $\pm$ 	0.155	&				&	Hya	&	Ros11	\\
LSPM J0409+1622	&		&	M5.5 V	&	B	&	Sma21	&	74092.6		&	28.769	 $\pm$ 	0.051	&	161.152	 $\pm$ 	0.075	&	2.339	 $\pm$ 	0.672	&	Hya	&	Ros11	\\
\noalign{\smallskip}        \noalign{\smallskip}																												
TYC 78--257--1	&		&	K3.0 V	&	A	&		&			&	26.974	 $\pm$ 	0.022	&	139.559	 $\pm$ 	0.028	&				&	Hya	&	Ros11	\\
RX J0422.4+0337	&	J04224+036	&	M3.5 V	&	B	&	Sma21	&	62796.5		&	27.846	 $\pm$ 	0.026	&	143.007	 $\pm$ 	0.039	&	9.22	 $\pm$ 	0.46	&	Hya	&	Ros11	\\
\noalign{\smallskip}        \noalign{\smallskip}																												
HD 27848$^d$	&		&	F5 V	&	AB	&	OCC 615	&			&	19.959	 $\pm$ 	0.026	&	103.388	 $\pm$ 	0.039	&				&	Hya	&	Ros11	\\
V991 Tau	&		&	K4 V	&	C	&		&	34929.6		&	18.356	 $\pm$ 	0.019	&	94.411	 $\pm$ 	0.025	&				&	Hya	&	Ros11	\\
V805 Tau	&	J04252+172	&	M3.5 V	&	DE	&	AST 4	&	51890.1		&	19.313	 $\pm$ 	0.193	&	110.653	 $\pm$ 	0.259	&				&	Hya	&	Ros11	\\
LP  415--881	&		&	M7.0 V	&	F	&		&	79117.5		&	21.204	 $\pm$ 	0.061	&	105.698	 $\pm$ 	0.088	&				&	Hya	&	Lod19	\\
\noalign{\smallskip}        \noalign{\smallskip}																												
LP 415--345	&	J04425+204	&	M3.0 V	&	Aab	&	Sta97	&			&	20.476	 $\pm$ 	0.022	&	97.452	 $\pm$ 	0.034	&				&	Hya	&	Gag18b	\\
LP 415--3051	&		&	M3.0 V	&	B	&	Sma21	&	34713.1		&	19.426	 $\pm$ 	0.020	&	91.262	 $\pm$ 	0.028	&				&	Hya	&	Ros11	\\
G2 3411054848866601472	&		&	M6.0 V	&	C	&	Sma21	&	83728.3		&	19.484	 $\pm$ 	0.118	&	93.825	 $\pm$ 	0.180	&				&	Hya	&	Lod19	\\
\noalign{\smallskip}        \noalign{\smallskip}																												
PM J05334+4809	&		&	M0.0 V	&	A	&		&			&	30.270	 $\pm$ 	0.018	&	66.932	 $\pm$ 	0.022	&				&		&		\\
PM J05341+4732 A	&	J05341+475	&	M2.5 V	&	B	&	EB21	&	75945.4		&	30.050	 $\pm$ 	0.027	&	69.013	 $\pm$ 	0.033	&	6.96	 $\pm$ 	0.52	&		&		\\
PM J05341+4732 B$^e$	&		&	M3.0 V	&	C	&	EB21	&	75899.1		&	30.039	 $\pm$ 	0.023	&	61.853	 $\pm$ 	0.028	&	5.20	 $\pm$ 	0.52	&		&		\\
UPM J0533+4809	&		&	M3.5 V	&	D	&	Sma21	&	4219.5		&	30.229	 $\pm$ 	0.235	&	65.011	 $\pm$ 	0.311	&				&		&		\\
\noalign{\smallskip}        \noalign{\smallskip}																												
1RXS J073138.4+455718	&		&	M3.0 V	&	Aab	&	Fou18	&			&	17.880	 $\pm$ 	0.416	&	93.776	 $\pm$ 	0.481	&				&		&		\\
1RXS J073101.9+460030	&	J07310+460	&	M4.0 V	&	B	&	Cif21	&	23780.3		&	18.141	 $\pm$ 	0.052	&	101.748	 $\pm$ 	0.059	&				&		&		\\
G3 975312928903090560	&		&	M4.5 V	&	C	&	Sma21	&	16738.6		&	18.388	 $\pm$ 	0.034	&	100.736	 $\pm$ 	0.042	&				&		&		\\
\noalign{\smallskip}        \noalign{\smallskip}																												
V869 Mon	&		&	K3 V	&	A	&		&			&	71.032	 $\pm$ 	0.024	&	286.810	 $\pm$ 	0.030	&				&	UMa	&	Tab17	\\
HD 61606 B	&		&	K7 V	&	B	&	BGH 3	&	815.63		&	70.992	 $\pm$ 	0.025	&	294.206	 $\pm$ 	0.031	&	1090	 $\pm$ 	231	&	UMa	&	Tab17	\\
GJ 282 C	&	J07361--031	&	M1.0 V	&	Cab	&	Pov09	&	6.2	273662.8018	&	70.275	 $\pm$ 	0.131	&	302.347	 $\pm$ 	0.173	&	3.766	 $\pm$ 	0.638	&	UMa	&	Tab17	\\
\noalign{\smallskip}        \noalign{\smallskip}																												
PM J13255+2738	&		&	M1.0 V	&	A	&		&			&	21.996	 $\pm$ 	0.019	&	71.210	 $\pm$ 	0.029	&				&		&		\\
PM J13260+2735 A	&	J13260+275	&	M3.0 V	&	B	&	Sma21	&	18493.6		&	21.868	 $\pm$ 	0.070	&	72.891	 $\pm$ 	0.109	&	26.54	 $\pm$ 	2.08	&		&		\\
PM J13260+2735 B	&		&	M2.5 V	&	C	&	KPP 3896	&	18343.6		&	22.030	 $\pm$ 	0.057	&	63.569	 $\pm$ 	0.092	&	21.74	 $\pm$ 	2.06	&		&		\\
\noalign{\smallskip}        \noalign{\smallskip}																												
HD 140232	&		&	A8 V	&	A	&		&			&	18.719	 $\pm$ 	0.041	&	82.169	 $\pm$ 	0.044	&				&		&		\\
G3 1197801408884577408	&		&	M3.5 V	&	B	&	DRS 17	&	126.52		&	18.642	 $\pm$ 	0.113	&	82.285	 $\pm$ 	0.167	&	8053	 $\pm$ 	1482	&		&		\\
StKM 1--1264	&	J15416+184	&	M1.5 V	&	C	&	TOK 302	&	12869.9		&	19.367	 $\pm$ 	0.139	&	91.885	 $\pm$ 	0.173	&	165.8	 $\pm$ 	25.7	&		&		\\
\noalign{\smallskip}        \noalign{\smallskip}																												
$\sigma$ CrB A	&		&	F6 V	&	Aab	&	Str03, Rag09	&	0.01		&	44.057	 $\pm$ 	0.046	&	282.061	 $\pm$ 	0.072	&				&		&		\\
$\sigma$ CrB B	&		&	G1 V	&	B	&	STF 2032	&	163.85		&	44.134	 $\pm$ 	0.018	&	301.273	 $\pm$ 	0.026	&	2567	 $\pm$ 	385	&		&		\\
$\sigma$ CrB C	&	J16139+337	&	M2.5 V	&	CD	&	STF 2032	&	11.5	14345.9663	&	44.267	 $\pm$ 	0.159	&	300.693	 $\pm$ 	0.241	&	12.28	 $\pm$ 	0.88	&		&		\\
\noalign{\smallskip}        \noalign{\smallskip}																												
HD 160269 A	&		&	G0 IV/V	&	AB	&	BU  962	&	9.02		&	69.283	 $\pm$ 	0.200	&	522.563	 $\pm$ 	0.334	&				&		&		\\
GJ 685	&	J17355+616	&	M0.5 V	&	C	&	LDS 2736	&	10561.5		&	69.892	 $\pm$ 	0.015	&	577.333	 $\pm$ 	0.023	&				&		&		\\
\noalign{\smallskip}        \noalign{\smallskip}																												
HD 230017 A	&		&	M0.0 V	&	A	&		&			&	53.423	 $\pm$ 	0.108	&	133.273	 $\pm$ 	0.161	&				&	Car	&	This work	\\
HD 230017 B	&	J18548+109	&	M3.5 V	&	B	&	VYS   8	&	70.68		&	53.644	 $\pm$ 	0.043	&	89.289	 $\pm$ 	0.063	&	6625	 $\pm$ 	637	&	Car	&	Gag18b	\\
PM J18542+1058	&		&	M4.0 V	&	C	&	This work	&	10009.5		&	53.838	 $\pm$ 	0.024	&	114.612	 $\pm$ 	0.034	&	38.59	 $\pm$ 	2.21	&	Car	&	This work	\\
\noalign{\smallskip}        \noalign{\smallskip}																												
AU Mic	&	J20451--313	&	M0.5 V	&	A	&		&			&	102.943	 $\pm$ 	0.023	&	456.998	 $\pm$ 	0.029	&				&	beta Pic	&	Cab09	\\
 AT Mic A	&	J20418--324	&	M4.5 V	&	B	&	LDS 720	&	45473.4		&	100.792	 $\pm$ 	0.073	&	484.794	 $\pm$ 	0.094	&				&	beta Pic	&	Ell14	\\
 AT Mic B	&		&	M4.5 V	&	C	&	LDS 720	&	20.62		&	101.972	 $\pm$ 	0.077	&	423.100	 $\pm$ 	0.097	&	14879	 $\pm$ 	1575	&	beta Pic	&	$\star$	\\
\noalign{\smallskip}        \noalign{\smallskip}																												
Wolf 1548	&	J22058--119	&	M0.0 V	&	A	&		&			&	38.616	 $\pm$ 	0.533	&	319.261	 $\pm$ 	1.369	&				&	Cas	&	Cab10	\\
LP 759--25	&		&	M6.0 V	&	B	&	WNO 57	&	59342.7		&	51.070	 $\pm$ 	0.054	&	322.495	 $\pm$ 	0.074	&	2.615	 $\pm$ 	0.227	&	Cas	&	$\star$	\\
\noalign{\smallskip}        \noalign{\smallskip}																												
G 29--19	&	J23175+063	&	M3.0 V	&	A	&		&			&	48.918	 $\pm$ 	0.027	&	302.148	 $\pm$ 	0.042	&				&		&		\\
G 28--50	&	J23161+067	&	M3.5 V	&	B	&	Sma21	&	36823.1		&	48.976	 $\pm$ 	0.026	&	304.894	 $\pm$ 	0.037	&	6.48	 $\pm$ 	0.38	&		&		\\
\noalign{\smallskip}        \noalign{\smallskip}																												
V368 Cep	&		&	G9 V	&	A	&		&			&	52.784	 $\pm$ 	0.014	&	215.918	 $\pm$ 	0.022	&				&	Col	&	$\star$	\\
HD 220140 B	&	J23194+790	&	M3.5 V	&	B	&	LDS 2035	&	206.38		&	52.840	 $\pm$ 	0.021	&	218.080	 $\pm$ 	0.036	&	3291	 $\pm$ 	548	&	Col	&	Gag18b	\\
LP 12--90	&	J23228+787	&	M5.0 V	&	C	&	MKR 1	&	18221.8		&	52.834	 $\pm$ 	0.030	&	217.441	 $\pm$ 	0.051	&	18.03	 $\pm$ 	2.89	&	Col	&	$\star$	\\
\noalign{\smallskip}        \noalign{\smallskip}																												
AF Psc	&	J23317--027	&	M4.5 V	&	A	&		&			&	28.631	 $\pm$ 	0.035	&	118.451	 $\pm$ 	0.051	&				&	Tuc-Hor/beta Pic	&	Kra14b	\\
2M J23301129--0237227	&	J23301--026	&	M6.0 V	&	B	&	CAB24	&	66833.9		&	21.982	 $\pm$ 	0.070	&	122.009	 $\pm$ 	0.110	&				&	Tuc-Hor/beta Pic	&	Alo15b	\\
\noalign{\smallskip}        \noalign{\smallskip}																												
HD 221503	&		&	K7 V	&	A	&		&			&	68.736	 $\pm$ 	0.027	&	405.450	 $\pm$ 	0.036	&				&		&		\\
GJ 1284	&	J23302--203	&	M3.0 V	&	Bab	&	Giz02, SHY 110	&	6.5	206051.1082	&	62.868	 $\pm$ 	0.076	&	375.234	 $\pm$ 	0.092	&				&		&		\\
GJ 897$^f$	&	J23327--167	&	M2.0 V	&	C	&	LDS 816	&	21894.8		&	64.8	 $\pm$ 	4.1	&	413.04	 $\pm$ 	3.75	&				&		&		\\
G3 2395220664463236992	&		&	M3.0 V	&	D	&	VOU 28	&			&		\ldots		&		\ldots		&				&		&		\\
\noalign{\smallskip}        \noalign{\smallskip}											
\end{longtable}
\tablefoot{
\tablefoottext{a}	{References for discovery --
Ben08: \cite{Ben08};
EB21: \cite{EB21};
Fou18: \cite{Fou18};
Giz02: \cite{Giz02};
Gri85: \cite{Gri85};
Pov09: \cite{Pov09};
Rag09: \cite{Rag09};
Sma21: \cite{Sma21};
Sta97: \cite{Sta97};
Str03: \cite{Str03};}
\tablefoottext{b}	{References for first assignation --
Alo15b: \cite{Alo15b};
Cab09: \cite{Cab09};
Cab10a: \cite{Cab10a};
Ell14: \cite{Ell14};
Gag18b: \cite{Gag18b};
Jan17: \cite{Jan17};
Kra14b: \cite{Kra14b};
Lod19: \cite{Lod19};
Ros11: \cite{Ros11};
Tab17: \cite{Tab17}.
The star symbol ($\star$) means the same SKG assignation as its physical companion, therefore sharing bibliographic reference. The list of abbreviations for the SKG can be found in Sect.~\ref{sssection:young}.}
\tablefoottext{c}	{LP~648--20: The $\sim$L0 companion %($\sim$ L0) 
reported by \cite{Ber10} based on lucky imaging  at 5.587\,arcsec is a background star ($\pi =$ 1.63\,mas).}
\tablefoottext{d}	{HD~27848: System dissected by \cite{Ben21}. Bona fide single star according to \cite{Bra23}.}
\tablefoottext{e}	{PM~J05341+4732\,B: Absent in the WDS but see \cite{Ans15} ($\rho=$ 2.33\,arcsec).}
\tablefoottext{f}	{GJ~897: Parallax and proper motions from Hipparcos \citep{van07}.}
}
\end{landscape}
}

